Combinatorial Selection with Costly Information

We consider a class of optimization problems over stochastic variables where the algorithm can learn information about the value of any variable through a series of costly steps; we model this information acquisition process as a Markov Decision Process (MDP). The algorithm's goal is to minimize the cost of its solution plus the cost of information acquisition, or alternately, maximize the value of its solution minus the cost of information acquisition. Such bandit superprocesses have been studied previously but solutions are known only for fairly restrictive special cases. We develop a framework for approximate optimization of bandit superprocesses that applies to arbitrary acyclic MDPs with a matroid feasibility constraint. Our framework establishes a bound on the optimal cost through a novel cost amortization; it then couples this bound with a notion of local approximation that allows approximate solutions for each component MDP in the superprocess to be composed without loss into a global approximation. We use this framework to obtain approximately optimal solutions for several variants of bandit superprocesses for both maximization and minimization. We obtain new approximations for combinatorial versions of the previously studied Pandora's Box with Optional Inspection and Pandora's Box with Partial Inspection; the less-studied Additive Pandora's Box problem; as well as a new problem that we call the Weighing Scale problem.

==> framework.tex <==
\section{Bandit Superprocesses and an Amortization Framework}\label{sec:framework}

\textcolor{blue}{
In this section, we formally introduce Bandit Superprocesses and establish our novel amortization framework, upon which we develop all of our results. In Section~\ref{sec:cis-definition}, we formally define our target class of problems, called Costly Information Superprocesses, and discuss the different settings we consider, such as minimization vs maximization, single-selection vs combinatorial etc. In Section~\ref{sec:mc-amortization}, we introduce our amortization framework for a special class of superprocesses over Markov chains, and recover well known optimality results for this setting, through the lenses of our amortization. In Section~\ref{sec:optimality-curves} we connect our amortization framework to the notion of optimality curves that was previously used to argue about the aforementioned optimality results. Finally, in Section~\ref{sec:mdp-amortization} we extend our amortization framework to bound the performance of the optimal algorithm for general Bandit Superprocesses; we note that while this result was previously known for the single-selection setting, we are the first to extend it into the combinatorial setting.
}





\subsection{Costly Information Superprocesses}\label{sec:cis-definition}
We begin by defining a single component of our algorithmic problem that involves learning information about a random variable through a series of costly steps. We represent this process as a \textit{Markov Decision Process} (henceforth, MDP). An MDP can be described by specifying its state space, the set of costly actions available in any state, and the distribution over states resulting from any action taken from any state. In the case of \textit{Costly Information MDPs}, states represent the information the algorithm has gained about the corresponding random variable. Accordingly, we associate each state with the conditional value distribution it represents. 

\begin{definition}[Costly Information MDP]
    A Costly Information MDP for a random variable $X$ is a tuple $\mc_X=(S, \sigma, A, c, \dist, V, T)$, where $S$ is a set of states, $\sigma\in S$ is the starting state, $A(\cdot)$ maps states to sets of actions, $c(\cdot)$ is a cost function mapping actions to costs, and $\dist$ is a transition matrix. For each pair of states $s,s'\in S$ and each action $a\in A(s)$, $\dist(s,a,s')\in [0,1]$ specifies the probability of transitioning to $s'$ upon taking action $a$ in state $s$; naturally, $\sum_{s'}\dist(s,a,s') = 1$. 
    
    Furthermore, $V(\cdot)$ is a function mapping states to distributions over values. $V(\sigma)$ is the (unconditional) distribution of $X$ and $V(s)$ is the posterior distribution of $X$ conditioned on being in state $s\in S$. As such, $V$ satisfies the usual rules of conditional probability: for all states $s\in S$ and all actions $a\in A(s)$, we have $V(s) = \sum_{s'} \dist(s,a,s') V(s')$. We also write $v(s) := \expect{V(s)}$. Finally, $T\subseteq S$ is the set of terminal states. Terminal states have only one action available, called the ``accept'' action. This accept action comes at no cost; results in a value of $v(s)$ at terminal state $s\in T$; and terminates the MDP. 
\end{definition}




When clear from the context, we will drop the subscript $X$. Furthermore, we call the process $\mc_X$ a {\em Costly Information Markov chain} if there is only one action (accept or advance) available at every state $s\in S$, i.e. whenever $|A(s)|=1$ for all $s\in S$.  Up next, we use these components in order to define the main class of algorithmic problems that this work considers, which we refer to as {\em Costly Information Superprocesses}.

\begin{definition}[Costly Information Superprocess]  

    We distinguish between the minimization and maximization versions of the problem.
    \begin{itemize}
        \item The minimization version of the Costly Information Superprocess problem (henceforth, min-CIS) is given by a ground set of $n$ random variables, $X_1, X_2, \cdots, X_n$; an upwards closed feasibility constraint $\feas\subseteq 2^{[n]}$; and a costly information MDP $\mc_i := \mc_{X_i}=(S_i, \sigma_i, A_i, c_i, \dist_i, V_i, T_i)$ for each variable $X_i$. 
        
        \item The maximization version of the Costly Information Superprocess problem (henceforth, max-CIS) is given by a ground set of $n$ random variables, $X_1, X_2, \cdots, X_n$; a downwards closed feasibility constraint $\feas\subseteq 2^{[n]}$; and a costly information MDP $\mc_i := \mc_{X_i}=(S_i, \sigma_i, A_i, c_i, \dist_i, V_i, T_i)$ for each variable $X_i$.
    \end{itemize}
    

    
\end{definition}

\paragraph{Algorithms and objective for minimization.} An algorithm (a.k.a. adaptive policy) for the min-CIS proceeds as follows. Let $S\subseteq [n]$ denote the set of indices of all terminated MDPs, that is, those where the accept action has been taken at one of their terminal states. Let $s_i$ denote the current state of the MDP $\mc_i$ at any point of time during the process. Initially $S=\emptyset$ and $s_i=\sigma_i$ for all $i$. The algorithm chooses at every step an index $i\in [n]\setminus S$ corresponding to a non-terminated MDP $\mc_i$ and an action $a_i\in A_i(s_i)$. It then follows the action at a cost of $c_i(a_i)$. If $a_i$ is the accept action (i.e. $s_i\in T_i$ is a terminal state), it adds $i$ to $S$, pays the value $v_i(s_i)$ and terminates the MDP $\mc_i$. Otherwise, it updates the state of $\mc_i$ to a new state drawn from the distribution $\dist(s_i, a_i, \cdot)$ and the states of all of the other MDPs $\mc_{i'}$ with $i'\ne i$, remain unchanged. The algorithm terminates as soon as $S\in \feas$. The cost of the algorithm is the expectation (over the randomness in the algorithm and the underlying processes) of the total cost of all actions undertaken by the algorithm until termination plus the values accrued from accept actions. The objective of the min-CIS problem is to find an algorithm with the minimum expected cost. 
    


\paragraph{Algorithms and objective for maximization.} An algorithm for the max-CIS proceeds in a similar manner with the key difference being feasibility and the termination condition. Once again let $S$ denote the set of indices of all terminated MDPs; initially $S=\emptyset\in\feas$. At every step, the algorithm chooses an index $i\in [n]\setminus S$ such that $S\cup\{i\}\in\feas$, and proceeds as before. The algorithm terminates when no index $i$ satisfies the feasibility constraint, that is, $S$ is a maximal feasible set. The utility of the algorithm is the expectation (over the randomness in the algorithm and the underlying processes) of the total reward accrued from accept actions {\em minus} the total cost of all actions undertaken by the algorithm until termination. The objective of the max-CIS problem is to find an algorithm with the maximum expected utility.

\color{blue}
\paragraph{Feasibility constraints.} The simplest and most natural type of feasibility constraints are \textit{single-selection constraints}, i.e. $\feas = \{\{i\} : i\in [n]\}$\footnote{For the max-CIS problem, we also include the empty set.}, where only one of the underlying MDPs can be terminated. Indeed, a large part of our framework will be developed with respect to these single-selection problems. However, we will also consider the case of more general \textit{combinatorial constraints}. Of particular interest will be the case of \textit{matroid constraints}, where each MDP corresponds to an element of some known matroid $\matroid$ and $\feas$ includes all subsets of elements that contain a basis of $\matroid$ (for the minimization version) or that form an independent set (for the maximization version). We refer to these problems as matroid-min-CIS and matroid-max-CIS, respectively. Note that the single-selection setting is a special case of the matroid setting.

Following the seminal work of~\citet{S17} and its follow up~\citep{GJSS19}, our results for the single-selection setting will seamlessly extend to any combinatorial setting (including matroid constraints) for which the underlying constraint admits an efficient {\em frugal} approximation algorithm. Intuitively, the class of frugal algorithms generalizes the concept of greedy algorithms. As such, this notion captures matroid constraints, set cover constraints and facility location constraints to name a few. We defer the details to Appendix~\ref{app:combinatorial} for ease of presentation.
\color{black}

\paragraph{Committing policies.} Observe that the choices of an algorithm for a CIS -- both the index of the MDP to move in and the action to take in that MDP -- can be made adaptively depending on the evolution of all $n$ MDPs in previous steps. The adaptivity of the optimal algorithm is the primary reason behind the computational hardness of these problem. In that sense, it is useful to consider a smaller class of simpler (and thus easier to optimize over) algorithms, which we call committing algorithms.

A committing policy $\pi$ for an MDP $\mc=(S, \sigma, A, c, \dist, V, T)$ maps every state $s\in S$ to a distribution $\pi(s)$ over actions in $A(s)$. An MDP $\mc$ coupled with a committing policy $\pi$ defines a Costly Information Markov chain, denoted $\mc^{\pi}$, where the single action available in every state is given by the distribution over actions specified by $\pi$. Observe that the states in $\mc^{\pi}$ are a subset of the states in $\mc$ and terminal states in $\mc$ continue to be terminal states in $\mc^{\pi}$. We use $\comset{\mc}$ to denote the set of all committing policies $\pi$ for MDP $\mc$.


A committing algorithm for a CIS is defined with respect of a tuple of committing policies $\Pi=(\pi_1, \cdots, \pi_n)$, one for each of the $n$ MDPs comprising the CIS. At every step, the algorithm chooses a feasible index $i$, samples an action from the distribution $\pi_i(s_i)$ and plays that action. 
Observe that although the (distribution over) action(s) taken by the algorithm is pre-chosen in every state, the algorithm can choose the index of the MDP to move in at every step adaptively based on the evolution of all $n$ MDPs in previous steps. Committing algorithms are therefore adaptive algorithms, although they are a simpler and smaller class relative to the class of all algorithms.

\textcolor{blue}{
\paragraph{Computational Considerations.} At the expense of blowing up the size of the state space and action set, we will assume that the sets of actions $A(s)$ and $A(s')$ are disjoint for $s\ne s'$, and furthermore that each state in the MDP $\mc_X$ is reached via a unique sequence of actions starting from $\sigma$; in other words, the state ``memorizes'' the sequence of actions taken to reach it and thus our MDPs have a tree-like structure. We will also assume that each MDP $\mc_X$ is a finite horizon MDP: there is a constant $H$ such that any state reached via a sequence of $H$ steps is a terminal state. Finally, we will only consider discrete random variables $X$ (and thus costly information MDPs of finite state and action spaces); we will say that an algorithm for a CIS is efficient if it runs in polynomial time to the size of the underlying MDPs. Nonetheless, our framework also extends to continuous random variables and infinite horizon MDPs; we defer these details to Appendix~\ref{app:contin}.
}

\bigskip
\textcolor{blue}{
For ease of presentation and to avoid repetition, in the main body of the paper we will establish our framework only for the \textbf{matroid-min-CIS}. \textbf{Since we refer to this constantly, we should give a nice name for it and make sure to state that instances will be denotes as $(\mc_1,\cdots , \mc_n , \feas)$ otherwise notation gets extremely repetitive in following sections.} Our entire framework extends to the maximization setting as-is, and we detail the differences in Appendix \ref{app:maxim}. Furthermore, our results seamlessly extend to a much richer family of combinatorial constraints, which we detail in Appendix \ref{app:combinatorial}.
}











\subsection{Amortized Surrogate Costs for Markov Chains}\label{sec:mc-amortization}

In this section we focus on the special case of the matroid-min-CIS where every MDP $\mc_i$ is a Markov chain. In this setting, an algorithm simply chooses a feasible index $i\in [n]$ at every step and advances $\mc_i$ along the unique action available. If $\mc_i$ is in a terminal state, the algorithm accepts it, pays the corresponding value and $\mc_i$ terminates, otherwise the state of $\mc_i$ evolves according to its transition matrix. 

Both the singe-selection and the (general) matroid versions of the min-CIS with Markov chains have been studied previously and it is well known that the optimal algorithm is an index policy. In particular, we associate every state $s_i\in S_i$ for $i\in [n]$ with an index.\footnote{This index is independent of the evolution of states in the algorithm, and depends solely on the description of the Markov chain.} The optimal algorithm simply advances the chain with the minimum index at every step. We will now describe a new simple proof of the optimality of index based policies based on a novel cost amortization process.

We begin with some notation. For a Costly Information Markov chain $\mc=(S, \sigma, A, c, \dist, V, T)$ and $s\in S$, we use $c(s)$ to denote the cost of the unique action $A(s)$. We use $R(s)\subseteq S$ to denote the set of all states reachable from $s\in S$ and $\ds(s) \subseteq T$ to denote the set of all {\em terminal} states reachable from $s$. Consider an algorithm that starts in the staring state $\sigma$ and advances the chain $\mc$ along the unique available action until it reaches a terminal state. For $s\in S$, let $p(s)$ denote the probability that the state $s$ is encountered during this process. Observe that by definition $p(s)=\sum_{t\in \ds(s)} p(t)$; $p(\sigma)=1$; and $p$ defines a probability distribution over the terminal states in $T$. We are now ready to define our notion of cost amortization.

\begin{definition}[Cost Amortization]
A cost amortization of a Markov chain $\mc=(S, \sigma, A, c, \dist, V, T)$ is a non-negative vector $b=\{b_{st}\}_{s\in S, t\in \ds(s)}$ with the property that $\sum_{t\in \ds(s)} p(t)b_{st}= p(s)c(s)$ for all states $s\in S$. Based on this amortization, we define:
\begin{itemize}
    \item The {\bf amortized cost} of a terminal state $t\in T$ as $W_b(t) := v(t) + \sum_{s:t\in \ds(s)} b_{st}$. 
    
    \item The {\bf surrogate cost} of the Markov chain $\mc$ as the random variable $W_{\mc,b}$ that takes on value $W_b(t)$ for $t\in T$ with probability $p(t)$.
    
    \item The {\bf index} of a state $s\in S$ of the Markov chain $\mc$ as $\ind_{\mc, b}(s)=\min_{t\in \ds(s)}W_b(t)$.
\end{itemize}


%We define the {\bf amortized cost} of a terminal state $t\in T$ as $W(t) := v(t) + \sum_{s:t\in \ds(s)} b_{st}$. 

%We say that a state $t\in T$ carries excess if $W(t)>v(t)$, and that a state $s\in S\setminus T$ carries excess if there exists $s'$ with $s\in R(S)$ and $t\in T(s)$ such that $b_{s't}>0$.

%The {\bf surrogate cost} of the Markov chain $\mc$ with respect to the amortization $b$ is the random variable $W_{\mc,b}$ that takes on value $W(t)$ for $t\in T$ with probability $p(t)$. The {\bf index} of a state $s\in S$ of the Markov chain $\mc$ with respect to the amortization $b$ is given by $\ind_{\mc, b}(s)=\min_{t\in \ds(s)}W(t)$.
\end{definition}

%\noindent
%The \textbf{total cost share} of a leaf $\ell\in\leafset{\mc}$ is given by $b_\ell := \sum_{e\in\advanceset{\mc}}b_{e\ell}$. We say that a leaf node $\ell\in \leafset{\mc}$ carries excess if $b_\ell>0$. We say that an advancement node $e\in\advanceset{\mc}$ carries excess if there are leaves in the subtree rooted at $e$ that contribute non-zero shares towards the cost of nodes upstream from $e$ (i.e. on the path from the root to $e$). Finally, we define the {\bf amortized cost} of a leaf node $\ell\in\leafset{\mc}$ as  $w_\ell := v_\ell + b_\ell$ and the \textbf{surrogate cost} of $\mc$ as the random variable $W_\mc$ that equals the amortized cost $w_\ell$ of a leaf node $\ell$ that is drawn from the distribution $\D_\mc$.

Observe that only terminal states carry amortized costs. The amortization essentially distributes the cost of every action across its downstream terminals. The surrogate cost of a Markov chain is the amortized cost of the random terminal state realized by running the chain until it terminates. The following lemma connects surrogate costs to optimal algorithms. 
\begin{lemma}
\label{lem:MC-lb}
    Consider a matroid-min-CIS with constraint $\feas$ over Markov chains $\mc_1, \cdots, \mc_n$, and let $b_i$ be any cost amortization of $\mc_i$ with surrogate cost $W_i := W_{\mc_i, b_i}$ for $i\in [n]$. Then,
    the expected cost of any algorithm for the matroid-min-CIS is at least $\expect{\min_{S\in\feas} \sum_{i\in S}W_i}$.
\end{lemma}

\color{blue}
\Cref{lem:MC-lb} has an intuitive interpretation. By definition, a cost amortization $b$ distributes the costs of all the actions into the terminal states, by increasing their values from $v(t)$ to $W_b(t)$. Now consider the setting where we substitute each Markov chain $\mc_i$ with its amortized version; since the amortized chains have $0$-cost actions, the optimal algorithm for the amortized instance will fully advance them and then accept the feasible subset of terminals of minimum amortized cost, at an expected cost of $\expect{\min_{S\in\feas} \sum_{i\in S}W_i}$. \Cref{lem:MC-lb} states that the amortized setting is easier than the original; this is due to the fact that while in the original setting action costs need to be paid in advance, in the amortized setting the algorithm only needs to pay the cost shares for the Markov chains it accepts, and thus its total cost is smaller in expectation. A detailed proof is given in Appendix~\ref{app:amortization}
\color{black}



We now exhibit a cost amortization and a corresponding algorithm that achieves the lower bound given in~\Cref{lem:MC-lb}, proving optimality. The {\em Water Filling} cost amortization is described algorithmically in a bottom-up fashion. Recall that each state in the Markov chain is associated with a unique sequence of actions that lead to it; let the length of this sequence denote the ``level'' of the state. We start from the terminal states, and define their total cost share to be equal to their value $v(t)$. We then proceed over non-terminal states in decreasing order of level. Each non-terminal state $s\in S$ distributes its total cost $c(s)$ across its downstream terminals $\ds(s)$ starting from the terminals with the lowest current total cost, until the equation $\sum_{t\in \ds(s)} p(t)b_{st}= p(s)c(s)$ is satisfied. A formal description of the Water Filling cost amortization can be found in Appendix~\ref{app:amortization}. 


We use $W^*_\mc$ to denote the Water Filling surrogate cost of the Markov chain $\mc$. We now define an index-based policy for the matroid-min-CIS problem based on the Water Filling amortization of the underlying Markov chains.

\begin{definition}[Water Filling Index Policy]\label{def:water-filling-index-policy}
    The Water Filling Index Policy for the matroid-min-CIS with constraint $\feas$ over Markov chains $\mc_1, \cdots, \mc_n$ is described as follows. Let $s_i$ denote the current state of $\mc_i$ for $i\in [n]$ and $\ind^*_i(s_i)$ denote the index of the state with respect to the Water Filling amortization. Let $S$ denote the set of indices of terminated Markov chains. The policy picks at every step $i^*=\argmin_{i\in \feas_S} \ind^*_i(s_i)$ and takes a step in $\mc_{i^*}$; here, $\feas_S \subseteq [n]\setminus S$ is the set of non-terminated Markov chains that increase the rank of $S$ if accepted.
\end{definition}

\textcolor{blue}{
In other words, the Water Filling index policy advances the Markov chains by order of the Water Filling amortization indices of their current states and never advances a chain once it has accepted a set of elements that span it. \textcolor{red}{not sure about terminology, I need to refresh my matroid definitions..} Furthermore, we note that the Water Filling amortization of a Markov Chain can be computed efficiently (with respect to the chain's size) and thus the same is true for the Water Filling Index Policy. The following theorem established optimality of the Water Filling Index Policy.}

\begin{theorem}
\label{thm:MC-opt}
    For any instance of the matroid-min-CIS with constraint $\feas$ over Markov chains $\mc_1, \cdots, \mc_n$, the expected cost of the Water Filling Index Policy is equal to the expected minimum surrogate cost, that is $\expect{\min_{S\in\feas} \sum_{i\in S}W^*_i}$. The Water Filling Index Policy is therefore optimal for this problem. 
\end{theorem}

\textcolor{blue}{
In essence, the index policy combined with the Water Filling amortization ensure that whenever an action $a$ is taken at some Markov chain and the realized updated state $s$ shares some of the (amortized) cost of $a$ through one of its terminal states $t\in T(s)$, the policy will keep advancing that chain. As a consequence, the policy will always pay (in expectation) the cost shares of any actions it takes, and thus its performance in the original and amortize settings will be the same, making the lower bound of~\Cref{lem:MC-lb} tight. The details are given in Appendix~\ref{app:amortization}.
}

\subsection{Local Games and Optimality Curves}\label{sec:optimality-curves}

We now connect the Water Filling amortization described above to the notion of \textit{optimality curves} for MDPs defined in the work of~\citet{W80} and its follow ups. We first define a ``local game'' for an MDP $\mc$.

\begin{definition}[Local Game]
    The {\bf local game} $(\mc, y)$ is a single-selection min-CIS with two MDPs, one of which is the MDP $\mc$. The second MDP, a.k.a. the outside option, is a deterministic option with a single state of value $y$ and a single ``accept'' action available. A policy for the local game advances $\mc$ for some (zero or non-zero) number of steps and either accepts the deterministic option $y$ or the value from $\mc$. Let $\optf_\mc(y)$ denote the expected cost of the optimal policy for $(\mc, y)$. We call $\optf_\mc$ the {\bf Optimality Curve} of the MDP $\mc$.
\end{definition}

\noindent
As a consequence of Theorem~\ref{thm:MC-opt} we obtain the following characterization:
\begin{fact}
    For any Markov chain $\mc$ and any $y\in \real$, 
    $\optf_\mc(y) = \expect{\min(y, W^*_\mc)}.$ %= \prob{y\le W^*_\mc}\cdot y + \prob{y> W^*_\mc}\cdot \expect{W^*_\mc | W^*_\mc < y}.\]
\end{fact}

\noindent
As a further consequence of this characterization, we observe that $1-\dd{y}{\optf_\mc(y)}$ is the CDF of the surrogate cost $W^*_{\mc}$.\footnote{In particular, let $H$ and $h$ denote the CDF and PDF of $W^*_\mc$ respectively, then we have $\optf_\mc(y) = y(1-H(y)) +\int_0^y zh(z)dz$, from which the statement follows by differentiating both sides.} This observation allows us to extend the definition of surrogate costs to arbitrary MDPs:
\begin{definition}
%[Water filling surrogate cost and index for MDPs]
[Water Filling surrogate cost for MDPs]
\label{def:mdp-wf}
    Let $\mc$ be an MDP with optimality curve $\optf_\mc$. The Water Filling Surrogate Cost for $\mc$ is the random variable $W^*_\mc$ generated by picking a value from the CDF $1-\dd{y}{\optf_\mc(y)}$. \textcolor{blue}{That is, $W^*_\mc$ is the random variable satisfying $\optf_\mc(y) = \expect{\min(y,W^*_\mc)}$ for all $y\in\real$.}
    
    %The Water Filling Index of the MDP is the minimum value in the support of this CDF.
\end{definition}
Unfortunately this definition does not give us insight into how the water filling surrogate costs relate to the structure of the MDP, or whether and how we can extend Lemma~\ref{lem:MC-lb} or Theorem~\ref{thm:MC-opt} to arbitrary MDPs. We will now address these issues by directly relating optimality curves to the water filling procedure.


\subsection{Water-filling and surrogate costs for MDPs}\label{sec:mdp-amortization}
\color{blue}
Let $\mc=(S, \sigma, A, c, \dist, V, T)$ be a Costly Information MDP and let $\optf_\mc$ denote its optimality curve. For any state $s\in S$, let $\mc_s$ denote the subprocess that starts in state $s$ and then has the same actions available in every downstream state as in the original MDP $\mc$. Let $\optf_s$ denote the optimality curve and $W^*_s$ denote the water filling surrogate cost for $\mc_s$ . We will also consider a subprocess that starts in state $s\in S$, follows action $a\in A(s)$, transitions according to $\dist$, and then has the same actions available in every downstream state as in the original MDP $\mc$; we call this subprocess $\mc_{sa}$ and use $T(sa)$, $\optf_{sa}$ and $W^*_{sa}$ to denote its set of terminal states, optimality curve and water filling surrogate cost, respectively. Note that $W^*_\mc = W^*_\sigma$.

Recall that advancing a Markov chain until a terminal state was reached generated a distribution over the terminal states of the chain. Likewise, any \textbf{sequence of actions} on an MDP also generates a distribution over (some) of its terminal states. The following key lemma connects the water filling surrogate costs of the subprocesses we defined through a novel notion of stochastic dominance.


\begin{lemma}
\label{lem:mdp-wf-char}
    For all states $s\in S$ and actions $a\in A(s)$, let $W^*_s$ and $W^*_{sa}$ be their corresponding water filling surrogate costs. Then, there exist functions $W_s: T(s)\mapsto \Delta(\real^+)$ and $W_{sa}: T(sa)\mapsto \Delta(\real^+)$ mapping the terminal states of $\mc_s$ and $\mc_{sa}$ to distributions over real numbers, such that:
    \begin{enumerate}

        \item {\bf (Action Independence.)} For \textbf{any} sequence of actions in the MDP $\mc_s$ (resp. $\mc_{sa}$), generating a distribution $\pi$ over $T(s)$ (resp. $T(sa)$), the random variable $W^*_s$ (resp. $W^*_{sa}$) is equivalent to sampling a terminal state $t\sim \pi$ and then sampling from $W_s(t)$ (resp. $W_{sa}(t)$). 
    
        \item {\bf (Cost Dominance.)} For all terminal states $t\in \ds(sa)$, $\expect{W_s(t)}\le\expect{W_{sa}(t)}$. 
    \end{enumerate}
\end{lemma}


The action independence condition states that each terminal state admits a distribution such that the water filling surrogate costs can be obtained by sampling a terminal state resulting from \textbf{any} sequence of actions on these subprocesses, and then sampling from this state's distribution. The cost dominance condition states that the expected cost assignment of any terminal state under $s$ lower bounds the expected cost of the same terminal under $sa$, for any action $a\in A(s)$. 

By inductively applying~\Cref{lem:mdp-wf-char} all the way to the starting state $\sigma$, and noting that $W^*_\sigma = W^*_\mc$, it essentially states that paying for a random instantiation of the water filling surrogate cost $W^*_\mc$ is preferable to paying the surrogate costs for any sequence of actions. With this intuition, the following counterpart of~\Cref{lem:MC-lb} follows easily from Lemma~\ref{lem:mdp-wf-char}. A formall proof is given in Appendix~\ref{app:amortization}.
\begin{theorem}
\label{thm:MDP-lb}
    For any instance of the matroid-min-CIS with constraint $\feas$ over MDPs $\mc_1, \cdots, \mc_n$, the expected cost of any algorithm is at least $\expect{\min_{S\in\feas}\sum_{i\in S} W^*_i}$, where $W^*_i$ denotes the water filling surrogate cost of $\mc_i$ as defined in Definition~\ref{def:mdp-wf}.
\end{theorem}



\color{black}

\color{magenta}
The rest of this section is dedicated towards proving~\Cref{lem:mdp-wf-char}. The proof follows by induction over the subprocesses $\mc_s$ in decreasing order of level. At the base case, we have the terminal states $t\in T$. For these states, we know that $f_t(y) = \min(y, v(t))$ and thus $W^*_t = v(t)$ with probability $1$; the corresponding mapping over $T(t) = \{t\}$ is $W_t(t):=v(t)$ and all the properties of~\Cref{lem:mdp-wf-char} trivially hold. Next, we will prove the claim for a state $s\in S$ and an action $a\in A(S)$, assuming (inductively) that the claim holds for all states $s'\in R(s)$ downstream from $s$.

\paragraph{Amortizing the action cost.} We first prove the conditions for the subprocess $\mc_{sa}$. Let $R(sa)$ be the set of states that are directly reachable from state $s$ after taking action $a$; formally, we define this set as $R(sa):=\{s'\in S: \dist(s,a,s')>0\}$. By definition of the optimality curves, we have
\begin{align*}
    f_{sa}(y) &= c(a) + \sum_{s'\in R(sa)}\dist(s,a,s')\cdot f_{s'}(y) \\
    &= c(a) + \sum_{s'\in R(sa)}\dist(s,a,s')\cdot \expect{\min\{y, W^*_{s'}\}} && \text{(By local optimality of $W^*_{s'}$)} \\
    &= c(a) + \expect{\min\{y, Z_{sa}\}}
\end{align*}
where $Z_{sa}$ is the random variable corresponding to first sampling a state $s'\sim \dist(s,a,\cdot)$ and then sampling from the distribution of the random variable $W^*_{s'}$. Next, let $g_{sa}$ be the solution to the equation
\[c(a) + \expect{\min\{y, Z_{sa}\}} = \expect{\min\{y, \max\{g_{sa},Z_{sa}\}\}};\]
in other words, $g_{sa}$ corresponds to the minimum value in the support of $Z_{sa}$ \textbf{after} we perform a water-filling amortization of the cost $c(a)$ onto the distribution of $Z_{sa}$. Thus, we conclude that the local game optimality condition is satisfied by the random variable $W^*_{sa}:= \max(g_{sa}, Z_{sa})$.

We will now argue that the action independence condition also holds. In particular, for any $t\in T(sa)$, consider the mapping $W_{sa}(t) := \max\{g_{sa}, W_{s'}(t)\}$ where $s'$ is the unique state $s'\in R(sa)$ such that $t\in T(s')$, and $W_{s'}(t)$ is the (action independent) mapping for terminal $t$ on $\mc_{s'}$; this exists by our induction hypothesis. By construction, the surrogate cost $W^*_{sa}$ corresponds to first sampling a state $s'\sim \dist(s,a,\cdot )$, then sampling a value from $W^*_{s'}$ and then returning the maximum of this value and $g_{sa}$. From the action independence condition on $W^*_{s'}$, this is the same as first sampling a state $s'\sim \dist(s,a,\cdot )$, then sampling a terminal $t\in T(s')$ by the distribution generated over any sequence of actions in $\mc_{s'}$ and then returning $\max\{g_{sa}, W_{s'}(t)\} =: W_{sa}(t)$. Since every sequence of actions on $\mc_{sa}$ starts with taking action $a$, we see that sampling from $W^*_{sa}$ is equivalent to sampling a terminal $t\in T(s)$ from the distribution generated by any arbitrary sequence of actions on $\mc_{sa}$ and then sampling from $W_{sa}(t)$, as desired.


\paragraph{Composing the different actions.} Next, we focus on state $s\in S$ and assume that the conditions are satisfied for all subprocesses $\mc_{sa}$ with $a\in A(s)$. 
By~\Cref{def:mdp-wf}, the random variable satisfying the local game optimality condition for $s$ is the water filling surrogate cost $W^*_s$, satisfying $f_s(y)=\expect{\min\{y, W^*_s\}}$. We will now need to to define a mapping over the terminal states $W_s: T(s)\mapsto \Delta(\real^+)$ that recovers this surrogate cost $W_s^*$ under any sequence on actions and also satisfies the cost dominance condition.


Note that for any fixed outside option $y$, we have the following principle of optimality:
\[\optf_s(y) = \min\left\{y, \min_{a\in A(s)} \optf_{sa}(y)\right\} = \min\left\{y, \min_{a\in A(s)} c(a) + \sum_{s'\in S} \dist(s,a,s') \optf_{s'}(y)\right\}.\]
By using the local game optimality on all subprocesses $M_{sa}$ with $a\in A(s)$, we re-write this as
\[\expect{\min\{y, W^*_s\}} = \min_{a\in A(s)}\left\{\expect{\min\{y, W^*_{sa}\}} \right\}\]

\begin{lemma}[Stochastic Dominance Lemma]
Let $X, Z$ be any two random variable for which $\expect{\min\{y, X\}} \leq \expect{\min\{y, Z\}}$ for all values of $y$. Then, there is a mapping $m: \mathrm{support}(Z) \mapsto \Delta(\mathrm{support}(X))$ from the support of $Z$ to distributions over the support of $X$ such that
\begin{enumerate}
    \item Sampling from $X$ is equivalent to sampling from a $z\sim Z$ and then sampling from $m(z)$.
    \item For all $z\in\mathrm{support}(Z)$, it holds that $\expect{m(z)}\leq z$.
\end{enumerate}
\end{lemma}

From the stochastic dominance lemma, combined with the action independence property on all $W^*_{sa}$, we see that for all $a\in A(S)$, sampling from $W^*_s$ is equivalent to sampling a terminal $t\in T(sa)$ from the distribution generated by an arbitrary sequence of actions on $\mc_{s}$ that starts with action $a$, then sample a value from the support of $W_{sa}(t)$ and finally sampling from the random mapping of this value that is defined by the stochastic dominance lemma. Furthermore, the cost dominance condition clearly holds. This completes the proof.

\color{black}




\begin{comment}


\begin{lemma}
\label{lem:mdp-wf-char}
    For all states $s\in S$ and actions $a\in A(s)$, there exist random variables $W^*_s$ and $W^*_{sa}$ that satisfy the following properties:
    \begin{enumerate}
        \item {\bf (Local Game Optimality.)} For all outside options $y$, the optimality curves for the corresponding local games are given by $\optf_s(y) = \expect{\min\{y, W^*_s\}}$ and $\optf_{sa}(y) = \expect{\min\{y, W^*_{sa}\}}$.

    
        \item {\bf (Action Independence.)} There exists a mapping from terminal states to distributions over cost assignments $W_s: T(s)\mapsto \Delta(\real^+)$ (resp. $W_{sa}: T(sa)\mapsto \Delta(\real^+)$) such that for \textbf{any} sequence of actions in the MDP $\mc_s$ (resp. $\mc_{sa}$), generating a distribution $\pi$ over $T(s)$ (resp. $T(sa)$), the random variable $W^*_s$ (resp. $W^*_{sa})$ is equivalent to sampling a terminal state $t\sim \pi$ and then sampling from $W_s(t)$ (resp. $W_{sa}(t)$).
        
        \item {\bf (Cost Dominance.)} For all terminal states $t\in \ds(sa)$, $\expect{W_s(t)}\le\expect{W_{sa}(t)}$. 
    \end{enumerate}
\end{lemma}
\color{black}


We note that the local game optimality condition simply states that $W^*_s$ and $W^*_{sa}$ will be the water filling surrogate costs for the subprocesses $\mc_s$ and $\mc_{sa}$ respectively, as defined in~\Cref{def:mdp-wf}. The action independence condition states that each terminal state admits a distribution such that the water filling surrogate costs can be obtained by sampling a terminal state resulting from \textbf{any} sequence of actions on these subprocesses, and then sampling from this state's distribution. The cost dominance condition states that the expected cost assignment of any terminal state under $s$ lower bounds the expected cost of the same terminal under $sa$, for any action $a\in A(s)$.


The following counterpart of~\Cref{lem:MC-lb} follows easily from Lemma~\ref{lem:mdp-wf-char}. We prove it formally in Appendix...
\begin{theorem}
\label{thm:MDP-lb}
    For any instance of the min-CIS over MDPs $\mc_1, \cdots, \mc_n$ with a \textcolor{red}{??} constraint, the expected cost of any algorithm is at least $\expect{\min_i W^*_i}$, where $W^*_i$ denotes the water filling surrogate cost of $\mc_i$ as defined in Definition~\ref{def:mdp-wf}.
\end{theorem}


\color{magenta}
The rest of this section is dedicated towards proving~\Cref{lem:mdp-wf-char}. The proof follows by induction over the subprocesses $\mc_s$ in decreasing order of level. At the base case, we have the terminal states $t\in T$. For these states, we know that $f_t(y) = \min(y, v(t))$ and thus $W^*_t = v(t)$ with probability $1$; the corresponding mapping over $T(t) = \{t\}$ is $W_t(t):=v(t)$ and all the properties of~\Cref{lem:mdp-wf-char} trivially hold. Next, we will prove the claim for a state $s\in S$ and an action $a\in A(S)$, assuming (inductively) that the claim holds for all states $s'\in R(s)$ downstream from $s$.

\paragraph{Amortizing the action cost.} We first prove the conditions for the subprocess $\mc_{sa}$. Let $R(sa)$ be the set of states that are directly reachable from state $s$ after taking action $a$; formally, we define this set as $R(sa):=\{s'\in S: \dist(s,a,s')>0\}$. By definition of the optimality curves, we have
\begin{align*}
    f_{sa}(y) &= c(a) + \sum_{s'\in R(sa)}\dist(s,a,s')\cdot f_{s'}(y) \\
    &= c(a) + \sum_{s'\in R(sa)}\dist(s,a,s')\cdot \expect{\min\{y, W^*_{s'}\}} && \text{(By local optimality of $W^*_{s'}$)} \\
    &= c(a) + \expect{\min\{y, Z_{sa}\}}
\end{align*}
where $Z_{sa}$ is the random variable corresponding to first sampling a state $s'\sim \dist(s,a,\cdot)$ and then sampling from the distribution of the random variable $W^*_{s'}$. Next, let $g_{sa}$ be the solution to the equation
\[c(a) + \expect{\min\{y, Z_{sa}\}} = \expect{\min\{y, \max\{g_{sa},Z_{sa}\}\}};\]
in other words, $g_{sa}$ corresponds to the minimum value in the support of $Z_{sa}$ \textbf{after} we perform a water-filling amortization of the cost $c(a)$ onto the distribution of $Z_{sa}$. Thus, we conclude that the local game optimality condition is satisfied by the random variable $W^*_{sa}:= \max(g_{sa}, Z_{sa})$.

We will now argue that the action independence condition also holds. In particular, for any $t\in T(sa)$, consider the mapping $W_{sa}(t) := \max\{g_{sa}, W_{s'}(t)\}$ where $s'$ is the unique state $s'\in R(sa)$ such that $t\in T(s')$, and $W_{s'}(t)$ is the (action independent) mapping for terminal $t$ on $\mc_{s'}$; this exists by our induction hypothesis. By construction, the surrogate cost $W^*_{sa}$ corresponds to first sampling a state $s'\sim \dist(s,a,\cdot )$, then sampling a value from $W^*_{s'}$ and then returning the maximum of this value and $g_{sa}$. From the action independence condition on $W^*_{s'}$, this is the same as first sampling a state $s'\sim \dist(s,a,\cdot )$, then sampling a terminal $t\in T(s')$ by the distribution generated over any sequence of actions in $\mc_{s'}$ and then returning $\max\{g_{sa}, W_{s'}(t)\} =: W_{sa}(t)$. Since every sequence of actions on $\mc_{sa}$ starts with taking action $a$, we see that sampling from $W^*_{sa}$ is equivalent to sampling a terminal $t\in T(s)$ from the distribution generated by any arbitrary sequence of actions on $\mc_{sa}$ and then sampling from $W_{sa}(t)$, as desired.


\paragraph{Composing the different actions.} Next, we focus on state $s\in S$ and assume that the conditions are satisfied for all subprocesses $\mc_{sa}$ with $a\in A(s)$. 
By~\Cref{def:mdp-wf}, the random variable satisfying the local game optimality condition for $s$ is the water filling surrogate cost $W^*_s$, satisfying $f_s(y)=\expect{\min\{y, W^*_s\}}$. We will now need to to define a mapping over the terminal states $W_s: T(s)\mapsto \Delta(\real^+)$ that recovers this surrogate cost $W_s^*$ under any sequence on actions and also satisfies the cost dominance condition.


Note that for any fixed outside option $y$, we have the following principle of optimality:
\[\optf_s(y) = \min\left\{y, \min_{a\in A(s)} \optf_{sa}(y)\right\} = \min\left\{y, \min_{a\in A(s)} c(a) + \sum_{s'\in S} \dist(s,a,s') \optf_{s'}(y)\right\}.\]
By using the local game optimality on all subprocesses $M_{sa}$ with $a\in A(s)$, we re-write this as
\[\expect{\min\{y, W^*_s\}} = \min_{a\in A(s)}\left\{\expect{\min\{y, W^*_{sa}\}} \right\}\]

\begin{lemma}[Stochastic Dominance Lemma]
Let $X, Z$ be any two random variable for which $\expect{\min\{y, X\}} \leq \expect{\min\{y, Z\}}$ for all values of $y$. Then, there is a mapping $m: \mathrm{support}(Z) \mapsto \Delta(\mathrm{support}(X))$ from the support of $Z$ to distributions over the support of $X$ such that
\begin{enumerate}
    \item Sampling from $X$ is equivalent to sampling from a $z\sim Z$ and then sampling from $m(z)$.
    \item For all $z\in\mathrm{support}(Z)$, it holds that $\expect{m(z)}\leq z$.
\end{enumerate}
\end{lemma}

From the stochastic dominance lemma, combined with the action independence property on all $W^*_{sa}$, we see that for all $a\in A(S)$, sampling from $W^*_s$ is equivalent to sampling a terminal $t\in T(sa)$ from the distribution generated by an arbitrary sequence of actions on $\mc_{s}$ that starts with action $a$, then sample a value from the support of $W_{sa}(t)$ and finally sampling from the random mapping of this value that is defined by the stochastic dominance lemma. Furthermore, the cost dominance condition clearly holds. This completes the proof.




    
\end{comment}




% Shuchi's draft of the MDP amortization
\begin{comment}
\subsection{Water-filling and surrogate costs for MDPs}

Let $\mc=(S, \sigma, A, c, \dist, V, T)$ be a Costly Information MDP and let $\optf_\mc$ denote its optimality curve. For $s\in S$, let $\mc_s$ denote the subprocess that starts in state $s$ and then has the same actions available in every downstream state as in the original MDP $\mc$. Let $\optf_s$ denote the optimality curve for $\mc_s$. We will also consider a subprocess that startes in state $s\in S$, follows action $a\in A(s)$, transitions according to $\dist$, and then has the same actions available in every downstream state as in the original MDP $\mc$; call this subprocess $\mc_{sa}$ and let $\optf_{sa}$ denote its optimality curve. 

We will now define the water filling amortization for the MDP $\mc$. %For $s\in S$ we denote the amortized cost of terminal state $t\in\ds(s)$ in the subprocess $\mc_s$ as $W^*_s(t)$ and the amortized cost of $t$ in the subprocess $\mc_{sa}$ as $W^*_{sa}(t)$. 
Our goal is to prove the following lemma.

\begin{lemma}
\label{lem:mdp-wf-char}
    For all $s\in S$ and $a\in A(s)$, there exist (random) assignments of amortized costs, $W^*_s(t)$ and $W^*_{sa}(t)$, to terminal states $t\in \ds(s)$ such that the following properties hold.
    \begin{enumerate}
        \item {\bf (Independence from actions.)} Consider any sequence of moves in the MDP $\mc_s$ (resp. $\mc_{sa}$) ending in a terminal state $t\in\ds(s)$ (resp. $t\in \ds(sa)$). The distribution of the (random) surrogate cost at the (random) terminal state resulting from this process is independent of the sequence of moves that generates it. We use $\pi_s$ (resp. $\pi_{sa}$) to denote this distribution and $W^*_s$ (resp. $W^*_{sa}$) to denote the random surrogate cost drawn from it.
        \item {\bf (Lower bounding of true costs.)} For all $s\in S$, $a\in A(s)$, and $t\in \ds(sa)$, $\expect{W^*_s(t)}\le\expect{W^*_{sa}(t)}$. 
        \item {\bf (Optimality in the local game.)} For all outside options $y$, $\optf_s(y) = \expectt{\pi_s}{\min\{y, W^*_s\}}$ and $\optf_{sa}(y) = \expectt{\pi_{sa}}{\min\{y, W^*_{sa}\}}$.
    \end{enumerate}
\end{lemma}

\noindent
The following counterpart of Lemma~\ref{lem:MC-lb} follows easily from Lemma~\ref{lem:mdp-wf-char}. We prove it formally in Appendix~\ref{}.
\begin{theorem}
\label{thm:MDP-lb}
    For any instance of the min-CIS over MDPs $\mc_1, \cdots, \mc_n$ with a \textcolor{red}{??} constraint, the expected cost of any algorithm is at least $\expect{\min_i W^*_i}$, where $W^*_i$ denotes the water filling surrogate cost of $\mc_i$ as defined in Definition~\ref{def:mdp-wf}.
\end{theorem}

\noindent
\color{magenta}
We devote the rest of this section to proving~\Cref{lem:mdp-wf-char} by induction over the subprocesses $\mc_s$ in decreasing order of level. At the base case, we have the terminal states $t\in T$. For these states, we know that $\optf_t(y) = \min\{y,v(t)\}$ and $W^*_t(t)=v(t)$. All of the properties in the lemma are trivially satisfied. Next, we will prove the claim for a state $s\in S$ and an action $a\in A(S)$, assuming (inductively) that the claim holds for all states $s'\in R(s)$ downstream from $s$.

\paragraph{Amortizing the action cost.} Let $R(sa)$ be the set of states that are directly reachable from state $s$ after taking action $a$; formally, we define $R(sa):=\{s'\in S: \dist(s,a,s')>0\}$. Observe that by the induction hypothesis, we have already defined surrogate costs $W^*_{s'}$ for all states $s'\in R(sa)$. Let $\pi_{s'}$ be the corresponding distributions over $t\in T(s')$ and $W^*_{s'}(\cdot)$ be the random assignments of amortized cost.


Furthermore, observe that by definition $T(sa) = \cup_{s'\in R(sa)} T(s')$. We define the distribution $\pi_{sa}$ as the distribution that first samples an $s'\in R(sa)$ according to $\dist(s,a,\cdot)$ and then samples $t\in T(s')$ from $\pi_{s'}$. For the random assignment of amortized costs, let
\[c(a) = \sum_{s'\in R(sa)}D(s,a,s')\sum_{t\in T(s')}\pi_{s'}(t)\sum_{\ell\in\mathrm{support}(W^*_{s'}(t))}p(\ell) \cdot b_\ell = \sum_{t\in T(s)} \pi_{sa}(t)\cdot ...\]
Define this as a water-filling amortization, this gives a formal definition of $\pi_{sa}$ and $W^*_{sa}$ and we need to show that the optimality curve is preserved through this amortization.

\newpage
and note that for any fixed outside option $y$, we have the following principle of optimality:
\[\optf_s(y) = \min\left\{y, \min_{a\in A(s)} \optf_{sa}(y)\right\} = \min\left\{y, \min_{a\in A(s)} c(a) + \sum_{s'\in S} \dist(s,a,s') \optf_{s'}(y)\right\}.\]

By the induction hypothesis, we have defined surrogate costs $W^*_{s'}$ for all states $s'\in R(s)$ downstream from $s$. 


Fix any action $a\in A(s)$. 


\end{comment}
\color{black}

==> grabvopen.tex <==
\section{Pandora's Box with Optional Inspection and Semi-Local Approximation}
\label{sec:gvo}

Finally, we consider \emph{Pandora's Box with Optional Inspection} (henceforth PBOI), a well-studied variant of the \emph{Pandora's Box} problem in which a box may be selected without first being opened. For brevity, we call selecting a box without first opening it ``grabbing'' the box. In the cost minimization (resp. reward maximization) setting, if the decision maker grabs a box, they pay (earn) the cost (value) inside of the box immediately, without ever having observed it. The availability of this extra action means that each box is now an MDP instead of a Markov chain, leading to a significantly more challenging optimization problem.

Most literature on PBOI is for single-item selection, as opposed to combinatorial variants. Study of it was initiated by \citet{GMS08}, who give a $4/5$-approximation for the maximization setting; and \citet{D18}, who characterized the solution to the single-box problem and proved certain conditions under which the Gittins policy remains optimal for single-item selection in the maximization setting (though the results naturally extend to the minimization setting). Beyond this results are separated by whether they are for the minimization or maximization setting. For the minimization setting, \citet{DS24} proved a composition theorem for a special case of local approximation (\cref{def:local-approx}) and used it to construct a committing policy with a $4/3$-approximation guarantee. In fact, their result extends beyond the single-item selection setting to the combinatorial Pandora's box setting studied by \citet{S17}, who proved that the Gittins policy is optimal for mandatory inspection combinatorial Pandora's box.

In the maximization setting, \citet{BK19} and \citet{GMS08} give approximation guarantees for committing policies. Furthermore, \citet{FLL22} and \citet{BC22} introduced polynomial time approximation schemes that for any $\varepsilon > 0$ compute a policy that is at least a $(1-\varepsilon)$-approximation. However, all of these results are for the single-item selection setting and do not extend to combinatorial settings such as matroid selection.

Currently, there is no known policy that achieves better than a $1/2$-approximation for matroid selection PBOI. Additionally, this $1/2$-approximation is somewhat uninteresting. As \citet{BK19} observe, the optimal policy that does not grab any box will attain half of the utility from boxes that the optimal doesn't open, and the optimal policy that only grabs boxes will attain half of the utility from boxes that the optimal grabs. Thus, uniformly randomizing between these policies will immediately give us a $1/2$-approximation.\footnote{%
    \Citet{BK19} make this observation in the single-item setting, but combining it with results of \citet{S17} generalizes it to the matroid setting.}

One might wonder whether one can use local approximation to break the $1/2$-approximation barrier. Alas, in the maximization setting, we cannot: there exist boxes for which we cannot do better than a local $(1/2+\varepsilon)$-approximation for any $\varepsilon > 0$ (\cref{lem:vanilla-local-hedging-bound-1/2}). Our contribution is a \emph{novel approach to break the $1/2$-approximation barrier} in the matroid selection setting, proving the following result.

\begin{theorem}\label{thm:gvo-approximation}
    There exists an efficient randomized committing policy, namely \cref{alg:semilocal_composition} with appropriately chosen probabilities, that achieves a $0.582$-approximation to the optimal adaptive policy for any instance of max-matroid-PBOI.
\end{theorem}

The key idea behind \cref{thm:gvo-approximation} is a refinement of local approximation, which we call \emph{semilocal approximation} (\cref{def:semilocal_approx}). Just as local approximations compose, we show in \cref{thm:semilocal_composition} that semilocal approximations similarly compose. We then show in \cref{thm:worst-case-semilocal-approx} that, unlike ordinary local approximation, all boxes admit a semilocal approximation that leads to a $0.582$-approximation. \Cref{thm:gvo-approximation} then follows immediately from \cref{thm:semilocal_composition, thm:worst-case-semilocal-approx}.

There are two prices we pay in refining local approximation to semilocal approximation. First, the definition as we state it currently is specific to PBOI, though it could perhaps be generalized to other MDP families in the future. Second, semilocal composition only holds for matroid selection problems, whereas past works showed results compatible with any frugal (roughly, ``greedy'') algorithm \citep{S17, GJSS19, DS24}. We believe this second obstacle may be fundamental.

% In \cref{sec:gvo:prelim} we introduce the model and review some existing results and bounds
% In \cref{sec:gvo:failure} we demonstrate that adapting the notion of local approximation used by [Ziv and Laura] to the maximization setting is insufficient to get an approximation better than $\frac{1}{2}$. In \cref{sec:gvo:composition} we introduce a refinement of local approximation designed specifically for PBOI, which we refer to as \emph{semilocal approximation}, since it is roughly local approximation along with an additional non-local aspect. We then prove that semilocal approximation composes in the desired way for the matroid selection setting. Finally, in \cref{sec:gvo:0.58} we bound the worst case semilocal approximation and show that it guarantees a $0.582$-approximation in the matroid selection setting.


% \textcolor{blue}{Problem definition}

% We will now consider another well-studied variant of the \textit{Pandora's Box} problem, where it is not mandatory to open a box in order to select in; instead, the decision maker can decide at any point to grab a closed box and pay its (yet unrealized) cost for the minimization setting (likewise, obtain its unrealized value for the maximization setting). This problem is known in the literature as \textit{Pandora's Box with Optional Inspection} (henceforth, PBOI). While very similar to the traditional Pandora's box problem, allowing optional inspections results to a much more challenging setting. Similarly to the partial inspection setting, the reason for that is that by offering a local decision of whether to grab or open a box to the decision maker, each box corresponds to an MDP rather than a Markov chain.

% \noindent\textcolor{blue}{---------------------------------------------------------------------------------------------------------------------------------------------}

%\textcolor{blue}{Literature review}

%The maximization version of Pandora's Box with Optional Inspection has been a very active line of research. Unfortunately, it has been shown that the optimal policy for this problem is indeed adaptive, and furthermore it does not inherit the simple properties of its mandatory inspection cousin \citep{D18}. In particular, finding the optimal policy is known to be an NP-complete problem \citep{FLL22, BC22}. Still, recent works have designed polynomial-time approximation schemes that can approximate the utility of the optimal policy up to a factor of $(1-\varepsilon)$ \citep{FLL22, BC22}. 

%A lot of work has also been done for committing policies \citep{GMS08,BK19,BC22}, with the best known approximation being $4/5$, and this is known to be tight. However, this result is nonconstructive. The resulting algorithm simply evaluates the expected value of all committing policies, then chooses the best one. While this approach is feasible for the single-item selection setting (where at most one box should be grabbed and thus the number of possible commitments in $n+1$), it cannot be applied in the more general combinatorial setting. For example, if the decision maker can choose up to $k$ rewards, then the number of committing policies is roughly $n^k$.

%To circumvent this issue, \citet{DS24} study the minimization variant of this problem and introduce the notion of local approximation in order to show that the MDPes corresponding to optional inspection boxes admit a $4/3$ local-approximation. Beyond a $4/3$-approximation for the single-item selection setting, this result naturally composes with any combinatorial setting that admits a frugal algorithm. As a consequence, it also implies a $4/3$-approximation for matroid selection for example.


% \noindent\textcolor{blue}{---------------------------------------------------------------------------------------------------------------------------------------------}

% \textcolor{blue}{Our results}


% In this work, we extend the results of \citet{DS24} to the maximization setting, for which combinatorial variants of Pandora's box with optional inspection have not been studied. In particular, we study local approximation for the MDPes corresponding to optional inspection boxes, that can be naturally composed to the combinatorial settings. Unfortunately, our vanilla version of local approximation cannot yield a better bound than~$1/2$.

%     Scratch: $m = 1 + n - \frac{1}{n^2}$.
%     When $y = 0$,
%     \(
%         \E{\max\{\alpha W^*, y\}} = \E{\alpha W^*} = \alpha m.
%     \)
    
%     If $y=m$,
%     \[
%         \E{\max\{\alpha W^*, y\}} = \max\{\E{\max\{\alpha W^\insp, m\}}, \alpha m\} = \E{\max\{\alpha W^\insp, m\}}
%     \]
%     And then for sufficiently large $n$ and all $\alpha \geq \frac{1}{2}$,
%     \begin{align*}
%         \E{\max\{\alpha W^\insp, m\}} &= \E_{X\sim\dist}{\max\{\alpha X, m\}} - \alpha c \\
%         &= (1-\frac{1}{n^2})m + \frac{1}{n^2}(\alpha n^3) - \alpha c \\
%         &= (1-\frac{1}{n^2})(1+n-\frac{1}{n^2}) + \alpha n - \alpha n + \alpha \\
%         &= \alpha + m(1-\frac{1}{n^2})\\
%         &= \alpha + 1 + n - \frac{1}{n}-\frac{2}{n^2}+\frac{1}{n^4}
%     \end{align*}

%     In particular, note that for sufficiently large $n$, $\E{\max\{W^\insp, m\}} = 1 + m(1-\frac{1}{n^2})$.

%     Thus, if we want to satisfy
%     \begin{equation*}
%         (1 - p) \E{\max\Bgp{W^\insp, y}} + p \max\Bgp{m, y}
%         \geq \E{\max\Bgp{\alpha W^*, y}}
%     \end{equation*}
%     at $y=0$ we have
%     \[
%         (1-p)(m-c) + pm \geq \alpha m
%     \]
%     and at $y=m$ we have (for sufficiently large $n$)
%     \[
%         (1-p)(1+m(1-\frac{1}{n^2})) + pm \geq \alpha + m(1-\frac{1}{n^2}).
%     \]
%     Rearranging both of these we get (again assuming $n$ is sufficiently large)
%     \begin{align*}
%         p &\geq \frac{\alpha m - m + c}{c} \\
%         p &\leq \frac{\alpha - 1}{\frac{m}{n^2}-1}
%     \end{align*}
%     respectively. Putting both of these together gets us that
%     \[
%         \alpha \leq \frac{(m (c - m + n^2))}{(-m^2 + c n^2 + m n^2)}.
%     \]
%     The RHS goes to $\frac{1}{2}$ as $n \to \infty$.
% \end{proof}

\subsection{PBOI Preliminaries}\label{sec:gvo:prelim}

Formally, we represent a box as a pair $\pbox = (\dist, c)$, where $\dist$ is a distribution over nonnegative values, and $c > 0$ is the opening cost. In order to learn the realization $X \sim \dist$, the decision maker can \emph{open} the box at a cost of~$c$. However, the decision maker can also select the box without first opening it. We call this latter action \emph{grab} to disambiguate it from selecting a previously opened box. See \cref{fig:gvo-states} for an illustration.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/gvo_states.png}
    \caption{A Pandora's box $\pbox = (\dist, c)$ under optional inspection is initially closed. In order to learn the value realization $X\sim\dist$, the decision maker can open it (at a cost of $c$), after which they can select it to accept its value~$X$. Alternatively, the decision maker can \emph{grab} the box, meaning select it without opening it, receiving the box's value~$X$ without paying any cost. Because $X$ is unknown whenever the box is being grabbed, for the purposes of expected value, receiving $X$ is equivalent to receiving $\E{X} = m$.}
    \label{fig:gvo-states}
\end{figure}

In this section, we at times consider Pandora's box problems under both \emph{optional inspection}, as illustrated in \cref{fig:gvo-states}, and \emph{mandatory inspection}, which is the traditional setting \citep{W79} that lacks the grab action. We use the same $\pbox = (\dist, c)$ notation for both, with context making it clear whether we are considering the box to be optional or mandatory inspection.

\begin{definition}[Indices and Surrogate Values for Pandora's Box]\label{def:gittins-and-backup-for-pb}
    Consider a box $\pbox = (\dist, c)$.
    \* The \emph{mean value} is $m = \E_{X \sim \dist}{X}$.
    \* The \emph{Gittins index} is~$g$, the solution to $c = \E_{X \sim \dist}{(X - g)^+}$.
    \* The \emph{backup index} is $h = \max\Bgp{m, h'}$, where $h'$ is the solution $c = \E_{X \sim \dist}{(h' - X)^+}$.\footnote{%
        Thanks to \cref{asm:pboi_normalized}, we will have $h = h'$ for most of the proofs, but the remaining lemmas in this subsection can be shown to hold even when $h = m > h'$. The key observation is that $W^* = m$ with probability~$1$ when $h = m$.}
    \* The \emph{opening surrogate value} is $W^\insp = \min\Bgp{X, g}$, where $X \sim \dist$ is the box's hidden value.
    \* The \emph{optimal surrogate value} is $W^* = \max\Bgp{\min\Bgp{X, g}, h} = \max\Bgp{W^\insp, h}$, where $X \sim \dist$ is the box's hidden value.
    \*/
    When the box in question is not clear from context, we clarify using subscripts, e.g. $g_1, g_2, \dots$ for the Gittins indices of boxes $\pbox_1, \pbox_2, \dots$.
\end{definition}

The reason for defining the surrogate values $W^\insp$ and $W^*$ as above is that they internalize the inspection cost of a box in exactly the right way such that the optimal reward for a single Pandora's box is equal to the choice between the surrogate value and the outside option \emph{in expectation}. This idea is formalized by the following lemma.
(\Cref{lem:prior-work-surrogate-costs-solve-one-item-subproblem} is a maximization version of \citet[Lemma~3.3]{DS24}.)

\begin{lemma}\label{lem:prior-work-surrogate-costs-solve-one-item-subproblem}
    For all $y \in \bbR$,
    \begin{align*}
        \E{\max\{W^\insp, y}\} &= \max\{\E_{X \sim \dist}{
                \max\{X,y\}
            }-c,
            y
        \} \\
        \E{\max\{W^*, y}\} &= \max\{\E_{X \sim \dist}{
                \max\{X,y\}
            }-c,
            y, m
        \}.
    \end{align*}
    These correspond to the optimal reward for a single Pandora's box with mandatory or optional inspection respectively.
\end{lemma}

We also review bounds from prior work on the optimal value achievable in matroid Pandora's box problems under mandatory inspection \citep[Theorem~1.5 and Lemma~2.1]{S17} and optional inspection \citep[Theorem~3.4]{DS24} (the latter translated from maximization to minimization).

\begin{lemma}
    Let $\instance = (B_1, \dots, B_n, \feas)$ be an instance of the max-matroid Pandora's box problem.
    \*[subenv]
    \* \label{thm:max_value_mand}
    Under \emph{mandatory} inspection, the optimal value, which is achieved by the frugal Gittins policy \citep{S17},\footnote{%
        The ``frugal Gittins policy'' referred to here and in \cref{alg:semilocal_composition} is essentially the water filling index policy specialized to Pandora's box, but for maximization instead of minimization. This is exactly the algorithm studied by \citet{S17}, so we use their ``frugal algorithm'' terminology.}
    is
    \[
        \E{\textnormal{value of optimal policy}} 
        = \E{\textnormal{value of frugal Gittins policy}} 
        = \E[\bigg]{\max_{S \in \feas} \sum_{i \in S} W^\insp_i}.
    \]
    \* \label{thm:max_value_opt}
    Under \emph{optional} inspection, the optimal value is at most
    \[
        \E{\textnormal{value of optimal policy}} \leq \E[\bigg]{\max_{S \in \feas} \sum_{i \in S} W^*_i}.
    \]
    \*/
\end{lemma}

Finally, following along the lines of \citet[Assumption~1]{D18}, we make an assumption for ease of presentation.

\begin{assumption}
    \label{asm:pboi_normalized}
    For all boxes $\pbox = (\dist, c)$ we consider, we assume the quantities from \cref{def:gittins-and-backup-for-pb} satisfy
    \[
        h \leq m.
    \]
    One can show that this further implies\footnote{%
        These follow from the following observations and plotting $m$, $y$, and $\E{\max\Bgp{X, y}} - c$ as functions of~$y$. (a)~$h = h'$ is the value of $y$ such that $m = \E_{X \sim \dist}{\max\Bgp{X, y}} - c$. (b)~$g$ is the value of $y$ such that $y = \E_{X \sim \dist}{\max\Bgp{X, y}} - c$. (c)~As a function of~$y$, the expression $\E_{X \sim \dist}{\max\Bgp{X, y}} - c$ has derivative in $[0, 1]$, and at $y = 0$, its value is $m - c$.}
    \[
        c \leq m \leq g.
    \]
    If a box~$\pbox$ fails this condition, we replace it with a \emph{normalized} box $\pbox_{\mathrm{norm}} = (m, 0)$, which trivially satisfies $h_{\mathrm{norm}} = m_{\mathrm{norm}} = g_{\mathrm{norm}} = m$.
\end{assumption}

This assumption says, roughly speaking, that every box has an open action that is sometimes worth taking.
We emphasize that boxes which fail \cref{asm:pboi_normalized} do not present an obstacle.
In fact, quite the opposite: the grab action is the only worthwhile action for such boxes.
See \citet[Section~2.2 and Appendix~S.4]{D18} for further discussion.
Rather than handling two cases throughout our presentation, we assume that all boxes are normalized in the way described in \cref{asm:pboi_normalized}.
Normalizing a box essentially removes the open action by replacing it with a ``no-op''.
Crucially, normalizing a box does not change the optimal surrogate value $W^*$, which is always~$m$ for boxes that violate \cref{asm:pboi_normalized}.
As such, the bound we employ on the expected value of the optimal policy (\cref{thm:max_value_opt}) remains true for the initial unnormalized system.


\subsection{Failure of Local Approximation for PBOI with Rewards}\label{sec:gvo:failure}

The relationship in \cref{lem:prior-work-surrogate-costs-solve-one-item-subproblem} allows us to rewrite the notion of local approximation introduced in \cref{def:local-approx} for the PBOI setting as follows.
(\Cref{def:vanilla-local-hedging-pboi} is a maximization version of \citet[Definition~4.2]{DS24}.)

\begin{definition}[Local $\alpha$-approximation for PBOI]
    \label{def:vanilla-local-hedging-pboi}
    Consider a box $\pbox = (\dist, c)$. We say the a probability $p \in [0,1]$ is a \emph{local $\alpha$-approximation} for $\pbox$ if for all $y$,
    \[
        (1-p)\E{\max\{W^\insp,y\}} + p\max\{m,y\} \geq \E{\max\{\alpha W^*, y\}}
    \]
\end{definition}
Intuitively, this is saying that if we commit to grabbing the box with probability $p$ and otherwise commit to inspecting it before opening it, we get a local $\alpha$-approximation. Unfortunately, this notion of local approximation only obtains a $(1/2)$-approximation in the worst case, as proven by the following lemma.

\begin{theorem}
    \label{lem:vanilla-local-hedging-bound-1/2}
    For all $\alpha > 1/2$, there exists a box that does not admit a local $\alpha$-approximation.
\end{theorem}

\begin{proof}
    For any $n \gg 1$, consider the box $\pbox^n$ where
        \[
            \dist = \begin{cases}
                1 & \text{w.p. } 1-\frac{1}{n^2} \\
                n^3 & \text{w.p. } \frac{1}{n^2} \\
            \end{cases}
        \]
    and $c = n-1$. Note that the mean of this distribution, $m$ is equal to $n+1-\frac{1}{n^2}$. \Cref{lem:prior-work-surrogate-costs-solve-one-item-subproblem} gets us that $\E{\max\{\alpha W^*, 0\}} = \alpha m$ and $\E{\max\{W^\insp, 0\}} = m - c$. Similarly, if $y=m$ then
        \[
            \E{\max\{\alpha W^*, y\}} = \max\{\E{\max\{\alpha W^\insp, m\}}, \alpha m\} = \E{\max\{\alpha W^\insp, m\}}
        \]
    and then a straightforward calculation gets us that for all $\alpha \geq \frac{1}{2}$ and sufficiently large $n$,
        \[
            \E{\max\{\alpha W^\insp, m\}} 
            = \E_{X\sim\dist}{\max\{\alpha X, m\}} - \alpha c
            = \alpha + m(1-\frac{1}{n^2}).
        \]
    Thus, if we want to satisfy
        \[
            (1 - p) \E{\max\Bgp{W^\insp, y}} + p \max\Bgp{m, y}
            \geq \E{\max\Bgp{\alpha W^*, y}}
        \]
    at $y=0$, we can plug in the quantities computed above and reorganize to get the bound $p \geq \frac{m(\alpha-1)}{c}+1$. Similarly, we can plug in our computed quantities when $y=m$ to get that when $n$ is sufficiently large and $\alpha \geq \frac{1}{2}$,
        \[
            p \leq \frac{\alpha - 1}{\frac{m}{n^2}-1}.
        \]
    Putting both of these bounds together, we get the following bound on $\alpha$,
        \[
            \alpha \leq \frac{m(c-m+n^2)}{mn^2+cn^2-m^2},
        \]
    which goes to $\frac{1}{2}$ from above as $n \to \infty$. Therefore, for any $\alpha > \frac{1}{2}$, we can choose $n$ large enough that $\pbox^n$ does not admit a local $\alpha$-approximation.
\end{proof}

To understand the behavior that leads to the worst case local $\alpha$-approximations, it will be illustrative to consider a box $\pbox^n$ for large $n$ as defined in the proof of \Cref{lem:vanilla-local-hedging-bound-1/2}. \Cref{fig:vanilla-local-hedging-bad-case-box} plots the value of grabbing versus inspecting as a function of the outside value $y$ for the box $\pbox^{20}$. As we can see, when $y$ is small we have a strong preference for grabbing the box, and when $y$ is larger we have a very slight preference to inspect the box. Looking at this plot makes it intuitively clear that the ``always grab'' policy performs quite well, since in the worst case there is only a small \emph{additive} sub-optimality factor. However, local $\alpha$-approximation requires a small \emph{multiplicative} sub-optimality factor, which, as the above proof demonstrates, the ``always grab'' policy does not achieve.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/gvo_plot.png}
    \caption{The red curve, $\max\{m,y\}$, represents the value from grabbing the box $\pbox^{20}$ (as defined in the proof of \cref{lem:vanilla-local-hedging-bound-1/2}). The blue curve, $\E{\max\{W^\insp, y\}}$, represents the value from inspecting the box $\pbox^{20}$. This box admits at most a local $0.537$-approximation. By considering $\pbox^n$ as $n \to \infty$, \cref{lem:vanilla-local-hedging-bound-1/2} shows that for all $\varepsilon > 0$, there exist boxes admit at most a local $(1/2 + \varepsilon)$-approximation.}%
    \label{fig:vanilla-local-hedging-bad-case-box}%
\end{figure}

To capture this intuition, in \cref{sec:gvo:composition}, we introduce \emph{semilocal $(\alpha, \beta)$-approximation} (\cref{def:semilocal_approx}), where $\alpha$ captures the multiplicative suboptimality while $\beta$ captures the additive suboptimality. We show that $(\alpha, \beta)$-semilocal approximations compose in the matroid selection setting leading to an overall $(\alpha-\beta)$-approximation (\cref{thm:semilocal_composition}). Then, in \cref{sec:gvo:0.58}, we show that all boxes admit a $(0.682, 0.1)$-semilocal approximation (\cref{thm:worst-case-semilocal-approx}), guaranteeing a $0.582$-approximation in the matroid selection setting and thus breaking the existing barrier of $1/2$.
% \Amit{if we discuss our results earlier, maybe they don't need to be here as well?}


\subsection{Semilocal Approximations and Their Composition}
\label{sec:gvo:composition}

\begin{definition}[Semilocal Approximation]
    \label{def:semilocal_approx}
    Consider a box $\pbox = (\dist, c)$. We say that a probability $p \in [0, 1]$ is a \emph{semilocal $(\alpha, \beta)$-approximation} for~$\pbox$ if for all~$y$,
    \begin{equation}\label{eq:def-semilocal-approx}
        (1 - p) \E{\max\Bgp{W^\insp, y}} + p \max\Bgp{m, y}
        \geq \E{\max\Bgp{\alpha W^*, y}} - p \beta m.
    \end{equation}
    If there exists a hedging probability that is a semilocal $(\alpha, \beta)$-approximation for the box~$\pbox$, then we say~$\pbox$ \emph{admits semilocal $(\alpha, \beta)$-approximation}.
\end{definition}
Rewriting \cref{eq:def-semilocal-approx} as
\[
    (1 - p) \E{\max\Bgp{W^\insp, y}} + p (\max\Bgp{m, y} + \beta m) 
        \geq \E{\max\Bgp{\alpha W^*, y}}.
\]
makes it clear that semilocal $(\alpha,\beta)$-approximation is basically a local $\alpha$-approximation where we have boosted the value attained from grabbing by an additive factor proportional to the mean. It is important that we do this only for grabbing—boosting the value of inspecting by an additive factor would lead to trivial guarantees when we compose semilocal approximations in the matroid selection setting.

\begin{algorithm}
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwFor{For}{For }{\unskip:}{}{}
    \SetKwIF{If}{ElseIf}{Else}{If}{\unskip:}{Else if}{Else}{}
    \SetKwComment{Comment}{}{}
    \DontPrintSemicolon
    \caption{Semilocal Approximation Composition Algorithm}
    \label{alg:semilocal_composition}
    \Input{%
        A matroid PBOI instance $\instance = (\pbox_1, \dots, \pbox_n, \feas)$ (normalized as described in \cref{asm:pboi_normalized}) \\
        A vector of probabilities $(p_1, \dots, p_n)$
    }
    \smallskip
    Relabel the boxes such that $m_1 \geq \dots \geq m_n$
    \;
    \smallskip
    $S^\grab \gets \{\}$
    \Comment*{\color{gray}\normalfont%
        set of boxes marked as ``grab''}
    \smallskip
    \For{\upshape$i \gets 1, \dots, n$}{%
        \smallskip
        \label{line:semilocal_composition:use_local}
        $L_i \gets \textbf{if } S^\grab \cup \{i\} \in \feas \textbf{ then } 1 \textbf{ else } 0$
        \Comment*{\color{gray}\normalfont%
            $L_i = 0$ means we never want to grab box~$i$}
        \smallskip
        Sample $K_i \gets \Bernoulli(p_i)$
        \Comment*{\color{gray}\normalfont%
            $K_i = 1$ means \emph{provisionally} mark box~$i$ ``grab''}
        \smallskip
        \If{\upshape$K_i = 1 \textbf{ and } L_i = 1$}{
            \smallskip
            $S^\grab \gets S^\grab \cup \{i\}$
            \Comment*{\color{gray}\normalfont%
                fully mark box~$i$ as ``grab''}
        }
    }
    \smallskip
    \label{line:semilocal_composition:commitment}
    Mark the boxes in $S^\grab$ as ``grab'' and the rest as ``open''
    \;
    \smallskip
    Run the frugal Gittins policy \citep{S17} on the resulting mandatory-inspection instance
    \;
\end{algorithm}

\begin{theorem}[Composition of Semilocal Approximations]
    \label{thm:semilocal_composition}
    Let $\alpha > \beta \geq 0$, let $\instance = (\pbox_1, \dots, \pbox_n, \feas)$ be a max-matroid-CICS instance, and let $(p_1, \dots, p_n)$ be a vector of probabilities such that $p_i$ is a semilocal $(\alpha, \beta)$-approximation for~$\pbox_i$.
    Then there exists a committing policy, namely \cref{alg:semilocal_composition}, that is an $(\alpha - \beta)$-approximation for the CICS instance~$\instance$.
\end{theorem}

\begin{proof}
    There are two main steps of the proof, each stated and proved in a lemma below.
    We express both steps in terms of the random variables
    \[
        W^\alg_i = \begin{cases}
            W^\insp_i & \text{if } K_i L_i = 0 \\
            m_i & \text{if } K_i L_i = 1,
        \end{cases}
    \]
    where $K_i$ and $L_i$ are as defined in \cref{alg:semilocal_composition}.
    One can think of $W^\alg_i$ as the surrogate value of box~$i$ conditional on the state of the algorithm at \cref{line:semilocal_composition:commitment}.
    \* The first step, \cref{thm:semilocal_composition:achieved}, is to express the value achieved by \cref{alg:semilocal_composition} in terms of~$W^\alg_i$.
    \* The second step, \cref{thm:semilocal_composition:comparison}, is to compare the resulting expression to an upper bound on the optimal value. This step uses the semilocal $(\alpha, \beta)$-approximation guarantee from \cref{def:semilocal_approx}, which gives us a relationship between $W^\alg_i$ and~$W^*_i$.
    \*/
    Combining the lemmas yields
    \[
        \E{\text{value achieved by \cref{alg:semilocal_composition}}}
        \geq \E[\bigg]{\max_{S \in \feas} \sum_{i \in S} \alpha W^*_i - \smashoperator{\sum_{i \in S^\grab}} \beta m_i},
    \]
    where $S^\grab$ is the set of boxes marked ``grab'' at \cref{line:semilocal_composition:commitment}, i.e. at the end of the algorithm.
    It remains only to relate the two terms on the right-hand side to the optimal expected value.
    \* \Cref{thm:max_value_opt} implies
    \[
        \E[\bigg]{\max_{S \in \feas} \sum_{i \in S} \alpha W^*_i} \geq \alpha \E{\text{value of optimal policy}}.
    \]
    % $\E[\big]{\max_{S \in \feas} \sum_{i \in S} \alpha W^*_i} \geq \alpha \E{\text{value of optimal policy}}$.
    \* Because \cref{alg:semilocal_composition} ensures $S^\grab \in \feas$ by construction, the following policy is feasible: ``Compute $S^\grab$ as in \cref{alg:semilocal_composition}, but then simply grab the boxes in $S^\grab$.'' This algorithm achieves value $\E[\big]{\sum_{i \in S^\grab} m_i}$, which means
    \[
        \E[\bigg]{\smashoperator[r]{\sum_{i \in S^\grab}} \beta m_i} \leq \beta \E{\text{value of optimal policy}}.
    \]
    % $\E[\big]{\sum_{i \in S^\grab} \beta m_i} \leq \beta \E{\text{value of optimal policy}}$.
    \*/
    Therefore, as desired, $\E{\text{value achieved by \cref{alg:semilocal_composition}}} \geq (\alpha - \beta) \E{\text{value of optimal policy}}$.
    % \[
    %     \E{\text{value achieved by \cref{alg:semilocal_composition}}}
    %     \geq (\alpha - \beta) \E{\text{value of optimal policy}}.
    %     \qedhere
    % \]
\end{proof}

\begin{lemma}
    \label{thm:semilocal_composition:achieved}
    For any max-matroid Pandora's box instance $\instance = (\pbox_1, \dots, \pbox_n, \feas)$ and any vector of probabilities $(p_1, \dots, p_n)$, the expected value achieved by \cref{alg:semilocal_composition} is
    \[
        \E{\textnormal{value achieved by \cref{alg:semilocal_composition}}}
        = \E[\bigg]{\max_{S \in \feas} \sum_{i \in S} W^\alg_i}.
    \]
\end{lemma}

\begin{proof}
    Consider running \cref{alg:semilocal_composition} through \cref{line:semilocal_composition:commitment}, but not further.
    All of the randomness thus far comes from the coin flips~$K_i$, and no boxes have been opened yet.
    This means that conditional on the coin flips~$K_i$, the expected value achieved is that of a \emph{mandatory-inspection} instance $\instance' = (\pbox'_1, \dots, \pbox'_n, \feas)$ whose $i$th box $\pbox'_i$ is defined as follows:
    \* If $K_i L_i = 0$ (marked ``open''), $\pbox'_i = (\dist_i, c_i)$, i.e. the box is the same as the original instance.
    \* If $K_i L_i = 1$ (marked ``grab''), $\pbox'_i = (m_i, 0)$, i.e. the box is free to open and always contains value~$m_i$.
    \*/
    Under instance~$\instance'$, box~$i$'s surrogate value is given by $W^\alg_i$, so
    \[
        \E{\text{value achieved by \cref{alg:semilocal_composition}} \given K_1, \dots, K_n}
        = \E[\bigg]{\max_{S \in \feas} \sum_{i \in S} W^\alg_i \given K_1, \dots, K_n}.
    \]
    The result then follows by the law of total expectation.
\end{proof}

\begin{lemma}
    \label{thm:semilocal_composition:comparison}
    Under the hypotheses of \cref{thm:semilocal_composition},
    \begin{equation}
        \label{eq:semilocal_composition:comparison}
        \E[\bigg]{\max_{S \in \feas} \sum_{i \in S} W^\alg_i}
        \geq \E[\bigg]{\max_{S \in \feas} \sum_{i \in S} \alpha W^*_i - \smashoperator{\sum_{i \in S^\grab}} \beta m_i},
    \end{equation}
    where $S^\grab$ refers to the value of the $S^\grab$ variable from \cref{alg:semilocal_composition} at \cref{line:semilocal_composition:commitment}.
\end{lemma}

\begin{proof}
    The outline of the proof is as follows.
    We begin with the left-hand side of~\cref{eq:semilocal_composition:comparison}.
    Then, for each box~$i$, we swap $W^\alg_i$ with $\alpha W^*_i$, and also subtract $\beta m_i$ if box~$i$ is marked ``grab''.
    Because each box admits a semilocal $(\alpha, \beta)$-approximation, each of these replacements only decreases the expression's expected value.
    After all $n$ replacements, we are left with the right-hand side of~\cref{eq:semilocal_composition:comparison}, as desired.
    This is the same strategy used by \citet[Theorem~5.4]{DS24}, but some careful conditioning is needed to account for the $\beta m_i$ subtractions.

    In order to notate the one-by-one replacement outlined above, let
    \begin{align*}
        W^{(j)}_i
        &= \begin{cases}
            W_i^\alg & \text{if } i \leq j \\
            \alpha W_i^* & \text{if } i > j,
        \end{cases}
        &
        U^{(j)}
        &= \max_{S \in \feas} \sum_{i \in S} W^{(j)}_i.
    \end{align*}
    Using this notation and recalling how $S^\grab$ is defined in \cref{alg:semilocal_composition}, we can rewrite our goal \cref{eq:semilocal_composition:comparison} as
    \[
        \E{U^{(n)}} \geq \E[\bigg]{U^{(0)} - \sum_{i = 1}^n \beta K_i L_i m_i}.
    \]
    Therefore, it suffices to show that for all $j \in \{1, \dots, m\}$,
    \begin{equation}
        \label{eq:semilocal_composition:suffices_1}
        \E{U^{(j)}}
        \geq \E[\bigg]{U^{(j - 1)} - \beta K_j L_j m_j}.
    \end{equation}

    We will show \cref{eq:semilocal_composition:suffices_1} using \cref{def:semilocal_approx}.
    But in order to do so, we need to express each side in terms of a maximum between $W^\alg_j$ or $\alpha W^*_j$ and a quantity that is independent of box~$j$'s value~$X_j$ and coin flip~$K_j$.
    We express the latter quantity in terms of
    \begin{align*}
        Y_{\neq j}
        &= \max_{S \in \feas : j \not\in S} \sum_{i \in S} W^{(j)}_i,
        &
        Z_{\neq j}
        &= \max_{S \in \feas : j \in S} \smashoperator[r]{\sum_{i \in S \setminus \{j\}}} W^{(j)}_i.
    \end{align*}
    These can both be seen as optimal total surrogate values achievable without box~$j$.
    The difference is that $Y_{\neq j}$ optimizes over sets that exclude~$j$, whereas $Z_{\neq j}$ optimizes over sets that include~$j$ (but still excludes box~$j$'s surrogate value from the sum).

    With the definitions of $Y_{\neq j}$ and $Z_{\neq j}$ in hand, we can express $U^{(j)}$ and $U^{(j - 1)}$ as
    \begin{align*}
        U^{(j)}
        &= \max\Bgp{Y_{\neq j}, Z_{\neq j} + W^\alg_j} = Z_{\neq j} + \max\Bgp{W^\alg_j, Y_{\neq j} - Z_{\neq j}},
        \\
        U^{(j - 1)}
        &= \max\Bgp{Y_{\neq j}, Z_{\neq j} + \alpha W^*_j} = Z_{\neq j} + \max\Bgp{\alpha W^*_j, Y_{\neq j} - Z_{\neq j}}.
    \end{align*}
    So to show \cref{eq:semilocal_composition:suffices_1}, it suffices to show
    \[
        \E{\max\Bgp{W^\alg_j, Y_{\neq j} - Z_{\neq j}}}
        \leq \E{\max\Bgp{W^\alg_j, Y_{\neq j} - Z_{\neq j}} - \beta K_j L_j m_j}.
    \]
    Letting $K_{< j} = (K_1, \dots, K_{j - 1})$, by the law of total expectation, it suffices to show
    \begin{equation}
        \label{eq:semilocal_composition:suffices_2}
        \E{\max\Bgp{W^\alg_j, Y_{\neq j} - Z_{\neq j}} \given K_{< j}, Y_{\neq j}, Z_{\neq j}}
        \leq \E{\max\Bgp{W^\alg_j, Y_{\neq j} - Z_{\neq j}} - \beta K_j L_j m_j \given K_{< j}, Y_{\neq j}, Z_{\neq j}}.
    \end{equation}
    The key to showing \cref{eq:semilocal_composition:suffices_2} is observing the following independence facts:
    \* $(K_j, X_j)$ is independent of $K_{< j}$. This is because the coin flips~$K_{< j}$ affect neither the coin flip~$K_j$ nor the box value~$X_j$.
    \* $(K_j, X_j)$ is conditionally independent of $(Y_{\neq j}, Z_{\neq j})$ given $K_{< j}$. This is because once $K_{< j}$ are fixed, the values $(Y_{\neq j}, Z_{\neq j})$ are a function of the values of boxes other than~$j$, and the box values are mutually independent.
    \*/
    The main obstacle to applying \cref{def:semilocal_approx} to \cref{eq:semilocal_composition:suffices_2} is that $W^\alg_j$ depends on $L_j$, which in turn depends on $K_{< j}$.
    Fortunately, we see from \cref{alg:semilocal_composition} that
    \[
        L_{\leq j} = (L_1, \dots, L_j) \text{ is a deterministic function of } K_{< j} = (K_1, \dots, K_{j - 1}).
    \]
    This is because for all~$i$, when executing \cref{line:semilocal_composition:use_local}, the only randomness the algorithm has used is the past coin flips~$K_{< i}$.
    So to show \cref{eq:semilocal_composition:suffices_2}, we split into cases based on whether $L_j = 0$ or $L_j = 1$.

    Suppose that $L_j = 1$.
    More precisely, suppose $K_{< j} = k_{< j}$, where $k_{< j}$ is any bit vector such that $K_{< j} = k_{< j}$ induces $L_j = 1$ in \cref{alg:semilocal_composition}.
    In this case, the coin flip~$K_j$ impacts whether we mark box~$j$ as ``grab'' or ``open'', so we will use the semilocal approximation guarantee from \cref{def:semilocal_approx}.
    By the assumption on $k_{< j}$ and the fact that $K_j \sim \Bernoulli(p_j)$ independently of $K_{< j}$,
    \[
        \E{K_j L_j \given K_{< j} = k_{< j}} = \E{K_j} = p_j.
    \]
    So, by \cref{def:semilocal_approx},
    \begin{align*}
        \E{\max\Bgp{W^\alg_j, y} \given K_{< j} = k_{< j}}
        &= (1 - p_j) \E{\max\Bgp{W^\insp_j, y}} + p_j \max\Bgp{m_j, y} \\
        &\geq \E{\max\Bgp{\alpha W^*_j, y}} - \beta p_j m_j \\
        &= \E{\max\Bgp{\alpha W^*_j, y} - \beta K_j m_j} \\
        &= \E{\max\Bgp{\alpha W^*_j, y} - \beta K_j L_j m_j \given K_{< j} = k_{< j}}.
    \end{align*}
    The fact that $(Y_{\neq j}, Z_{\neq j})$ is conditionally independent of $(K_j, X_j)$ given $K_{< j}$ completes the proof of \cref{eq:semilocal_composition:suffices_2} on the event $L_j = 1$.

    Suppose now that $L_j = 0$.
    In this case, we mark box~$j$ as ``open'' regardless of the coin flip~$K_j$, so instead of using \cref{def:semilocal_approx}, we will show that marking box~$j$ as ``open'' does not lose any any potential value.
    Specifically, we will show the following:
    \*[(a)] For all $y \geq h_j$, we have $\E{\max\Bgp{W^\insp_j, y}} = \E{\max\Bgp{W^*_j, y}}$.
    \* If $L_j = 0$, then $Y_{\neq j} - Z_{\neq j} \geq m_j$.
    \*/
    Together with the fact that $m_j \geq h_j$ (\cref{asm:pboi_normalized}), facts~(a) and~(b) imply that for any $k_{< j}$ such that $K_{< j} = k_{< j}$ induces $L_j = 0$ in \cref{alg:semilocal_composition},
    \begin{align*}
        \E{\max\Bgp{W^\alg_j, Y_{\neq j} - Z_{\neq j}} \given K_{< j} = k_{< j}}
        &= \E{\max\Bgp{W^\insp_j, Y_{\neq j} - Z_{\neq j}} \given K_{< j} = k_{< j}} \\
        &= \E{\max\Bgp{W^*_j, Y_{\neq j} - Z_{\neq j}} \given K_{< j} = k_{< j}} \\
        &\geq \E{\max\Bgp{\alpha W^*_j, Y_{\neq j} - Z_{\neq j}} \given K_{< j} = k_{< j}} \\
        &= \E{\max\Bgp{\alpha W^*_j, Y_{\neq j} - Z_{\neq j}} - \beta K_j L_j m_j \given K_{< j} = k_{< j}},
    \end{align*}
    which completes the proof of \cref{eq:semilocal_composition:suffices_2} on the event $L_j = 0$.
    It remains only to show (a) and~(b).
    For~(a), observe that if $y \geq h_j$, then $y_j = \max\Bgp{h_j, y_j}$, so
    \[
        \E{\max\Bgp{W^\insp_j, y}}
        = \E{\max\Bgp{W^\insp_j, h_j, y}}
        = \E{\max\Bgp{W^*_j, y}}.
    \]
    For~(b), we will show that if $L_j = 0$, then $Y_{\neq j} \geq m_j + Z_{\neq j}$.
    Let
    \* $B^Z \in \argmax_{S \in \feas : j \in S} \sum_{i \in S \setminus \{j\}} W^{(j)}_i$ be a maximizing basis in the definition of $Z_{\neq j}$,
    \* $S^\grab_{< j} = S^\grab \cap \{1, \dots, j - 1\}$ be the boxes marked ``grab'' before the $i = j$ for loop iteration, and
    \* $B^\grab$ be $S^\grab_{< j}$ extended to a basis by elements of $B^Z$, so that $S^\grab_{< j} \subseteq B^\grab \subseteq S^\grab_{< j} \cup B^Z$.
    \*/
    Because $L_j = 0$, we have $S^\grab_{< j} \cup \{j\} \not\in \feas$, which means $j \not\in B^\grab$.
    But $j \in B^Z$ by definition, so $j \in B^Z \setminus B^\grab$.
    By the basis exchange property, there exists $k \in B^\grab \setminus B^Z$ such that the following is a basis:
    \[
        B^Y = (B^Z \setminus \{j\}) \cup \{k\}.
    \]
    But $B^\grab \setminus B^Z \subseteq S^\grab_{< j}$, which means $W^{(j)}_k = m_k \geq m_j$.
    This means
    \[
        Y_{\neq j}
        \geq \smashoperator{\sum_{i \in B_Y}} W^{(j)}_i
        = m_k + \smashoperator{\sum_{i \in B_Z \setminus \{j\}}} W^{(j)}_i
        \geq m_j + \smashoperator{\sum_{i \in B_Z \setminus \{j\}}} W^{(j)}_i
        = m_j + Z_{\neq j}.
        \qedhere
    \]
\end{proof}

% \subsection*{\Ziv{Old proof}}

% \begin{proof}[Proof for special case of single-item selection]
%     \Ziv{Generalize to matroids, then add appropriately generalized lemmas. Also distinguish better between $L_i$ and the event $W^\alg_i = W^\hedge_i$. Probably do so by introducing separate indicators for ``chose this option in hedging'' and ``decided to use hedging at all''.}
%     We are not going to immediately flip coins for all the boxes.
%     Instead, we will go through the boxes one by one, flipping coins as we go.
%     Specifically, we order boxes such that $m_1 \geq \dots \geq m_n$, and go through the boxes in order from $1$ to~$n$.
%     When focusing on box~$i$, we assign it a label $L_i$, along with an associated surrogate value $W^\alg_i$, as follows.
%     \* If we have already labeled a box $j < i$ as grab, i.e. if $L_j = 1$, then we label box~$i$ as inspect, i.e. we set $L_i = 0$ and set $W^\alg_i = W^\insp_i$.
%     \* Otherwise, we label box~$i$ randomly according to its hedging probability~$p_i$, i.e. we set $L_i \sim \Bernoulli(p_i)$ to be the assigned label and set $W^\alg_i = W^\hedge_i$.
%     Note that $L_i$ and $W^\alg_i = W^\hedge_i$ are \emph{not} independent (either overall or conditionally on this case occurring).
%     \*/

%     From here, there are two steps.
%     First, we need to find the expected value achieved by this algorithm.
%     A corollary of \cref{thm:fancy_lh_single:condition} implies this value is
%     \[
%         \E{\max\Bgp{W^\alg_1, \dots, W^\alg_n}}.
%     \]
%     Second, we need to show that this value is at least $\alpha - \beta$ times the optimum.
%     Repeatedly applying \cref{thm:fancy_lh_single:replace} (see below) shows
%     \begin{align*}
%         \E{\max\Bgp{W^\alg_1, \dots, W^\alg_n}}
%         &\geq \alpha \E{\max\Bgp{W^*_1, \dots, W^*_n}} - \beta \E{m_1 L_1 + \dots + m_n L_n} \\
%         &\geq \alpha \E{\max\Bgp{W^*_1, \dots, W^*_n}} - \beta m_1,
%     \end{align*}
%     where the second line follows because $L_1 + \dots + L_n \leq 1$ and $m_1 \geq \dots \geq m_n$.
%     The result then follows from \cref{thm:max_value_opt:single} and the fact that the optimum is clearly at least~$m_1$.
% \end{proof}

% \begin{lemma}
%     \label{thm:fancy_lh_single:condition}
%     The expected value achieved by the algorithm given $L_1, \dots, L_n$ is
%     \[
%         \E[\big]{W^\alg_1 \vee \dots \vee W^\alg_n \given L_1, \dots, L_n}.
%     \]
% \end{lemma}

% \begin{proof}
%     The values $L_1, \dots, L_n$ are determined according to some randomized procedure that is independent of the values $X_1, \dots, X_n$, because the procedure occurs prior to opening any boxes.
%     The expected value given $L_1, \dots, L_n$ is thus the expected value of a mandatory-inspection problem with the following possibly modified ``primed'' boxes.
%     \* If $L_i = 0$, i.e. box~$i$ is labeled inspect, then it is not modified, i.e. $c_i' = c_i$ and $X_i' = X_i$.
%     \* If $L_i = 1$, i.e. box~$i$ is labeled grab, then we modify it to $c_i' = 0$ and $X_i' = \mu_i$ with probability~$1$.
%     \*/
%     One can check that $(W^\insp_i)' = W^\alg_i$ given $L_i$, so the result follows from \cref{thm:max_value_mand:single}.
% \end{proof}

% The following lemma uses subscripts like ``${<} i$'' to denote vectors, e.g. $L_{< i} = (L_1, \dots, L_{i - 1})$.

% \begin{lemma}
%     \label{thm:fancy_lh_single:replace}
%     \begin{align*}
%         \MoveEqLeft
%         \E[\big]{\max\gp{W^\alg_{< i}} \vee W^\alg_i \vee \alpha \max\gp{W^*_{> i}} \given L_{< i}}
%         \\ &
%         \geq \E[\big]{\max\gp{W^\alg_{< i}} \vee \alpha W^*_i \vee \alpha \max\gp{W^*_{> i}} - \beta \mu_i L_i \given L_{< i}}.
%     \end{align*}
% \end{lemma}

% \begin{proof}
%     There are two cases to consider, depending on whether some box $j < i$ has already been labeled grab.

%     If $\max(L_{< i}) = 0$, i.e. all boxes are labeled inspect so far, then $W^\alg_i = W^\hedge_i$ and $L_i \sim \Bernoulli(p_i)$. The result then follows from the assumption that $i$ admits fancy local $(\alpha, \beta)$-approximation.

%     If instead $\max(L_{< i}) = 1$, i.e. a box $j < i$ is labeled grab, then $W^\alg_i = W^\insp_i$ and $L_i = 0$.
%     Because we order the boxes such that $\mu_1 \geq \dots \geq \mu_n$, the box~$j$ labeled grab has mean $\mu_j \geq \mu_i$.
%     But (by assumption of box~$i$ not being a trivial always-grab box) we have
%     \[
%         \mu_j \geq \mu_i \geq h_i,
%     \]
%     so for all~$r$,
%     \begin{align*}
%         \E{W^\insp_i \vee \mu_j \vee r}
%         &= \E{W^\insp_i \vee h_i \vee \mu_j \vee r} \\
%         &= \E{W^*_i \vee \mu_j \vee r} \\
%         &= \E{W^*_i \vee \mu_j \vee r - \beta \mu_i L_i} \\
%         &\geq \E{\alpha W^*_i \vee \mu_j \vee r - \beta \mu_i L_i},
%     \end{align*}
%     as desired.
%     The last two lines follow because $L_i = 0$ and $\alpha \leq 1$, respectively.
% \end{proof}


\subsection{Breaking the $1/2$ Barrier with Semilocal Approximation}
\label{sec:gvo:0.58}

\begin{lemma}\label{lem:semilocal-alpha-beta-approximation-for-fixed-beta}
    Consider a box $\pbox$ satisfying \cref{asm:pboi_normalized}. For all $\beta \in \bbR$ there exists a $p \in [0,1]$ that is a semilocal $(\alpha(\beta), \beta)$-approximation for $\pbox$ where
    \[
        \alpha(\beta) = \begin{cases}
            \frac{1}{1+\frac{c}{m}-\beta\frac{c}{m-c}} & \text{if } 1 \geq \frac{1}{1+\frac{c}{m}-\beta\frac{c}{m-c}} > 0 \\
            1 & \textnormal{otherwise.}
        \end{cases}
    \]
    Moreover, the $p$ that achieves this is $p=\alpha(\beta)\frac{c}{m}$.
\end{lemma}

% \noindent
% \emph{Remark.} Note that $\frac{m}{c}-1 \geq \beta$ is equivalent to $1+\frac{c}{m}-\beta\frac{c}{m-c} \leq \frac{c}{m}$.

\begin{proof}
    To simplify notation we denote $\alpha(\beta)$ as $\alpha$ throughout the proof. Proving this lemma amounts to showing that this $\alpha$ and $\beta$ satisfy \cref{eq:def-semilocal-approx},
    \[
        (1 - p) \E{\max\Bgp{W^\insp, y}} + p \max\Bgp{m, y}
        \geq \E{\max\Bgp{\alpha W^*, y}} - p \beta m
    \]
    for all $y \geq 0$. This is equivalent to showing that
    \[
        f(y) = (1 - p) \E{\max\Bgp{W^\insp, y}} + p \max\Bgp{m, y} - \E{\max\Bgp{\alpha W^*, y}} + p \beta m
    \]
    satisfies $f(y) \geq 0$ for all $y \geq 0$. We will first show that it is sufficient to check that $f(0) \geq 0$ and that $f(y) \geq 0$ for $y \geq m$. It follows from \cref{def:gittins-and-backup-for-pb} that at all values $y$ for which $f'(y)$ is defined, it is equal to
    \[
        (1-p) \prob{y \geq W^\insp} + p \ind(y > m) - \ind(y > \alpha h)\prob{y > \alpha W^\insp}.
    \]
    Observe that
    \begin{itemize}
        \item if $y < \alpha h < m$, then $f'(y) \geq 0$,
        \item if $\alpha h < y < m$, then since $\alpha \leq 1$, we must have $f'(y) \leq 0$.
    \end{itemize}
    Thus a global minimum of $f(y)$ must be at $y = 0$ or on $y \geq m$, so it is sufficient to check that \cref{eq:def-semilocal-approx} is satisfied when $y=0$ and $y \geq m$. When $y=0$, \cref{eq:def-semilocal-approx} reduces to
    \begin{equation*}
        (1-p)(m-c)+pm \geq \alpha m-p\beta m.
    \end{equation*}
    which holds for the values of $\alpha$ and $p$ given in the lemma.
    When $y \geq m$, \cref{eq:def-semilocal-approx} reduces to
    \begin{equation}\label{eq:semilocal-approx-suff-inequality-y>m}
        (1-p) \E{\max\Bgp{W^\insp, y}} + py
        \geq \E{\max\Bgp{\alpha W^*, y}} - p \beta m = \alpha\E{\max\Bgp{W^\insp, \frac{y}{\alpha}}} - p \beta m 
    \end{equation}
    where the last equality follows from the fact (\cref{lem:prior-work-surrogate-costs-solve-one-item-subproblem}) that $\E{\max\Bgp{\alpha W^*, y}} = \max\{\E{\max\Bgp{\alpha W^\insp, y}}, \alpha m\}$. The slope of $\E{\max\{W^\insp, y\}}$ is bounded above by $1$, so 
    \[
        \alpha\E{\max\Bgp{W^\insp, \frac{y}{\alpha}}} \leq \alpha \E{\max\Bgp{W^\insp, y}} + \alpha \left(
            \frac{y}{\alpha} - y
        \right).
    \]
    Applying this bound to \cref{eq:semilocal-approx-suff-inequality-y>m}, we find that \cref{eq:semilocal-approx-suff-inequality-y>m} holds if,
    \begin{equation}\label{eq:semilocal-approx-suff-inequal-y>m-after-bound}
        (\alpha+p-1) (\E{\max\Bgp{W^\insp, y}}-y)
        \leq p \beta m. 
    \end{equation}
    Since the slope of $\E{\max\{W^\insp, y\}}$ is bounded above by $1$, it must be that $\E{\max\Bgp{W^\insp, y}}-y$ is maximized at $y=0$ where it is equal to $m - c$, so \cref{eq:semilocal-approx-suff-inequal-y>m-after-bound} holds if,
    \[
        (\alpha+p-1) (m-c)
        \leq p \beta m. 
    \]
    Observe that if $p = \alpha\frac{c}{m}$, we can rewrite this inequality as
    \[
        \alpha\left(1 + \frac{c}{m} - \frac{c}{m-c}\beta \right) \leq 1,
    \]
    which is satisfied by the $\alpha$ given in the lemma.
\end{proof}

\begin{theorem}\label{thm:worst-case-semilocal-approx}
    For any box $\pbox$ satisfying \cref{asm:pboi_normalized}, if $\beta = \frac{1}{10}$, the $p$ given in \cref{lem:semilocal-alpha-beta-approximation-for-fixed-beta} is an $(\alpha, \beta)$-semilocal approximation for $\pbox$ with $\alpha \geq 0.682$.
\end{theorem}

\begin{proof}
    \Cref{lem:semilocal-alpha-beta-approximation-for-fixed-beta} guarantees that for $\beta = \frac{1}{10}$, there is some $p \in [0,1]$ that is an $(\alpha, \beta)$-semilocal approximation for $\pbox$ with
    \[
        \alpha = \begin{dcases}
            \frac{1}{1+\frac{c}{m}-\frac{c}{10(m-c)}} & \text{if } 1 \geq \frac{1}{1+\frac{c}{m}-\frac{c}{10(m-c)}} > 0 \\
            1 & \text{otherwise.}
        \end{dcases}
    \]
    It is straightforward to verify (using a computer algebra system or numerical solver) that since $\frac{c}{m}\in[0,1]$, $1 {\bigm/} \gp[\big]{1+\frac{c}{m}-\frac{c}{10(m-c)}} \geq 0.682$ when $1 \geq 1 {\bigm/} \gp[\big]{1+\frac{c}{m}-\frac{c}{10(m-c)}} > 0$.
\end{proof}

% \begin{proof}
%     \emph{this is a first messy write up to get everything on the page}

%     ~
    
%     \noindent
%     We need to find $\alpha < 1, \beta > 0$, and $0 \leq p \leq 1$ that satisfy the following inequality for all $r \geq 0$,
%     \[
%         p\E{\max (W^\insp, r)} + (1-p)\max(r,m) \geq 
%         \left(
%             \E{\max (\alpha W^\insp, r)} \vee \alpha m
%         \right)
%         -(1-p)\beta m.
%     \]
%     Note that when $r = 0$, this reduces to
%     \begin{equation}\label{eq:semilocal-approx-r=0-ineq}
%         p(m - c) + (1-p)m \geq \alpha m -(1-p)\beta m.
%     \end{equation}
%     since $\E{W^\insp} = m - c$.
%     Similarly, when $r \geq m$,
%     \[
%         p\E{\max (W^\insp, r)} + (1-p)r \geq \alpha \E{\max (W^\insp, \frac{r}{\alpha})} -(1-p)\beta m.
%     \]
%     Since the slope of $\E{\max(W^\insp, r)}$ is bounded above by $1$, we get the following bound,
%     \[
%     \alpha \E{\max (W^\insp, \frac{r}{\alpha})} \leq \alpha \E{\max (W^\insp, r)} + \alpha (\frac{r}{\alpha} - r).
%     \]
%     So by plugging this into the earlier inequality and reorganizing, we get the following (sufficient) inequality,
%     \[
%         (\alpha- p)(\E{\max (W^\insp, r)} - r) \leq (1-p)\beta m.
%     \]
%     Since $\E{\max (W^\insp, r)}$ has slope no greater than $1$ and equals $m - c$ at $r=0$, it must be that ${\E{\max (W^\insp, r)} - r \leq m - c}$, so it is sufficient to have
%     \begin{equation}\label{eq:semilocal-approx-r>m-ineq}
%     (\alpha- p)(m - c) \leq (1-p)\beta m.
%     \end{equation}

%     Thus we have two inequalities that together ensure our desired inequality holds when $r=0$ or $r \geq m$. We claim that this is sufficient to ensure that the inequality holds for all $r$.

%     Define
%     \[
%         f(r) = p\E{\max (W^\insp, r)} + (1-p)\max(r,m) -
%         \E{\max (\alpha W^\insp, r)} \vee \alpha m
%         + (1-p)\beta m
%     \]
%     and note that we need $f(r) \geq 0$ for all $r \geq 0$. Observe that the derivative (where it exists) is
%     \[
%         f'(r) = p\prob{r > W^\insp} + (1-p)\ind(r > m)-\ind(r > \alpha h)\prob{r > \alpha W^\insp}.
%     \]
%     Using this expression we see that,
%     \begin{itemize}
%         \item If $r < \alpha h$, then $r < m$ and $f'(r) = p\prob{r > W^\insp} \geq 0$.
        
%         \item If $\alpha h < r  < m$, then $f'(r) = p\prob{r > W^\insp} - \prob{r > \alpha W^\insp}\leq 0$ since $\alpha < 1$.
        
%         \item If $m < r$, then $f'(r) =  p\prob{r > W^\insp} + (1 - p) - \prob{r > \alpha W^\insp}$, which can be positive or negative. 

%         % \item if $m < r$ and $\alpha g < r$, then $\prob{r >\alpha W^\insp} = 1$ and $f'(r) \leq 0$.
%     \end{itemize}
%     Thus the global minimum of $f(r)$ is either at $r=0$ or on $r \geq m$.

%     We can rewrite \ref{eq:semilocal-approx-r=0-ineq} as
%     \[
%         \alpha m - p(m-c) - (1-p)m \leq (1-p)\beta m
%     \]
%     and then subtract \ref{eq:semilocal-approx-r>m-ineq} to get
%     \[
%         p\leq 1-\alpha \frac{c}{m} .
%     \]
%     Let $p = 1-\alpha \frac{c}{m}$ and plug into \ref{eq:semilocal-approx-r=0-ineq} to get
%     \[
%         1 \geq \alpha(1+\frac{c}{m}-\frac{\beta}{\frac{m}{c}-1}).
%     \]
%     If the RHS is negative, this is a trivial inequality. If it is positive, we must have
%     \[
%         \frac{1}{1+x-\frac{\beta}{\frac{1}{x}-1}} \geq \alpha
%     \]
%     where $x = \frac{c}{m}$. 
%     Observe that this bound is strictest when the LHS is minimized. It is straightforward to check that the unique minimum on $0 \leq x \leq 1$ occurs when $x=1-\sqrt{\beta}$. Thus we have the sufficient condition,
%     \[
%         \frac{1}{2-\sqrt{\beta} - \frac{\beta}{\frac{1}{1-\sqrt{\beta}}-1}} \geq \alpha
%     \]
%     and therefore
%     \[
%         \frac{1}{2-\sqrt{\beta} - \frac{\beta}{\frac{1}{1-\sqrt{\beta}}-1}} - \beta \geq \alpha - \beta.
%     \]
%     The maximum of the LHS can be found using a computer algebra system or numerical solver to be approximately $0.5814$ when $x \approx 0.101$.
% \end{proof}

==> new_introduction_1.tex <==
\section{Introduction - Old Version}\label{sec:intro}






%\noindent \Dimitris{1. Real-life motivating examples.}


Consider a biotechnology company investing in multiple drug discovery projects. Each individual project can involve a multitude of decisions with uncertain outcomes. Typically, very few projects will make it to trials and FDA approval, at which point they can begin to yield rewards for the company. The company needs to determine how to distribute resources across these projects without knowing upfront which one will succeed and to what extent. Similarly, many decision making problems call for upfront investment in information acquisition (such as how much reward a project will generate) before optimizing over multiple options (such as which project to seek FDA approval for). Other examples include an oil company's search for a good drilling site; a construction company exploring different design ideas for a project; a manufacturer performing market research before determining which products to make and in what quantity, etc.

%Consider a biotechnology company investing in multiple drug discovery projects. Each individual project can involve a multitude of decisions with uncertain outcomes. Typically very few projects will make it to trials and FDA approval at which point they can begin to yield rewards. Therefore, the company needs to determine how to distribute resources across these projects without knowing upfront which one will succeed and to what extent. Similarly, many decision making problems call for upfront investment in information acquisition (such as how much reward a project will generate) before optimizing over multiple options (such as which project to seek FDA approval for). Some other examples include an oil company's search for a good drilling site; a construction company exploring different design ideas for a project; a manufacturer performing market research before determining which products to make and in what quantity, etc.

%As a toy example of costly information acquisition in the context of optimization, consider what we call the {\em Weighing Scale} problem. The algorithm is presented with $n$ alternatives with unknown costs, $X_1, \cdots, X_n$, of which it needs to pick a cheap one. Each cost $X_i$ is distributed independently according to a known distribution. The only way the algorithm can learn any further information about the $X_i$'s is to use a weighing scale at the additional cost of $1$ per use: for any index $i$ and target $t$, the weighing scale returns $\mathbbm{1}[X_i \le t]$. What information, if any, should the algorithm gather before making its selection so as to minimize the expected cost of the chosen alternative plus the number of weighings?


%\noindent \Dimitris{2. Definition of CICS.}

This work aims to model such decision making scenarios by introducing a family of problems that we call {\em Costly Information Combinatorial Selection} (henceforth, CICS). In CICS, our goal is to select a subset of $n$ alternatives with stochastic values under some feasibility constraint. We can obtain information about the value of any individual alternative through a sequence of costly actions tailored to that alternative. We model this information acquisition process for alternative $i$ as a Markov decision process (henceforth, MDP) $\mc_i$. The MDPs $\mc_1, \cdots, \mc_n$ are independent: the states in $\mc_i$ correspond only to the information we have learned thus far about alternative $i$ and the costly actions available in $\mc_i$ only reveal further information about $i$. %At any point, we can obtain information about the value of any individual alternative by selecting one (of possibly many) costly actions tailored to it; the set of available actions depends only on the information we have already acquired for this alternative. 
In the minimization version of the problem our objective is to minimize the total value of the chosen alternatives plus the cost of information acquisition. In the maximization version we maximize the total value of the chosen subset minus the cost of information acquisition. 



%In this paper we study a class of problems that we call {\em Costly Information Combinatorial Selection} (henceforth, CICS), of which Weighing Scale is an example. Our goal is to pick a subset of $n$ alternatives with stochastic values satisfying a feasibility constraint. We can obtain information about the value of any individual alternative through a sequence of costly actions tailored to that alternative. In the minimization version of the problem our objective is to minimize the total value of the chosen alternatives plus the cost of information acquisition. In the maximization version we  maximize the total value of the chosen subset minus the cost of information acquisition. 

%\noindent \Dimitris{3. CICS have two main challenges: local and global decision making.}



The algorithmic challenge of CICS stems from two different levels of decision making that influence each other. In particular, at each step, a policy (a.k.a. an algorithm) needs to select which of the $n$ alternatives to explore (global decision making); as well as which alternative-specific action to take in order to explore it (local decision making). At any point of time, the policy can terminate by accepting any feasible subset of alternatives for which the underlying MDPs have reached a terminal (sink) state. In general, these choices are made adaptively, based on all the information that was obtained in previous steps.


%The algorithmic challenge of CICS stems from two levels of decision-making that influence each other -- which alternative to explore in each step; as well as how to explore the chosen alternative (e.g. which target values $t$ to use in the Weighing Scale setting). A policy can, in general, make these choices adaptively based on the information obtained on previous steps.

%\noindent \Dimitris{4. Absence of local decision making $\rightarrow$ easy. An example is Weitzman's Pandora's Box + extensions.}

CICS is well understood in the special case where no local decision making is required -- in particular,  there is a unique way to explore each alternative at any point of time, and the MDP $\mc_i$ is simply a Markov chain. A classic example is the Pandora's Box problem, introduced by \cite{W79}. Here, each alternative is hidden inside a closed box; the goal is to select a single alternative; the algorithm can observe the value of the alternative by opening, a.k.a. ``inspecting'', each box at a cost; and any alternative must be inspected before being selected. Pandora's Box admits an astonishingly simple optimal algorithm: each box is assigned an index based on its cost and value distribution; for minimization, boxes are inspected in increasing\footnote{For the maximization version of the problem, boxes are opened in decreasing order of index.} order of index until the algorithm finds a value that is smaller than all remaining indices and accepts that value. Essentially, the indices capture all of the salient information about each individual box and can be used by the algorithm to determine the (optimal) fixed exploration order. Interestingly, this optimality structure extends to a large class of feasibility constraints over Pandora's Boxes: \cite{S17} showed that Weitzman's indices and the corresponding greedy ordering algorithm achieve approximate optimality for essentially all selection problems that admit greedy-style (a.k.a. frugal) approximation algorithms. Furthermore, the same index-based optimality structure extends to general Markov chains \citep{DTW03,GJSS19}.
%instances where each box requires multiple stages of inspection before the algorithm can select it. 


%A classic example of the CICS is Weitzman's Pandora's Box problem. Here each alternative is hidden inside a closed box; the goal is to select a single alternative; the algorithm can observe the value of the alternative by opening, a.k.a. ``inspecting'', each box at a cost; and any alternative must be inspected before being selected. Pandora's Box admits an astonishingly simple optimal algorithm: each box is assigned an index based on its cost and value distribution; for minimization, boxes are inspected in increasing\footnote{For the maximization version of the problem, boxes are opened in decreasing order of index.} order of index until the algorithm finds a value that is smaller than all remaining indices and accepts that value. The indices do not depend on the algorithm's stochastic trajectory; the order of information acquisition is therefore non-adaptive. Essentially, {\em the indices capture all of the salient information about each individual box} that can then be used by the algorithm to determine the order in which to explore the boxes. 

%Interestingly, this optimality structure extends to a large class of feasibility constraints over Pandora's Boxes: \cite{S17} showed that Weitzman's indices and the corresponding greedy ordering algorithm achieve approximate optimality for essentially all selection problems that admit greedy-style (a.k.a. frugal) approximation algorithms.

%\noindent \Dimitris{5. Presence of local decision making $\rightarrow$ hard.}

In the presence of local decision making, the algorithm has multiple modes of information acquisition available for each alternative and the landscape changes significantly. For example, if inspection of a Pandora's Box becomes optional, that is, if the algorithm is allowed to select an alternative without observing its value, the optimal algorithm no longer inspects the boxes in a fixed order and computing the optimal solution is NP-hard \citep{FLL22}. In general, the optimal policy for CICS no longer exhibits the same structural properties as in the special case of Markov chains, and it is not possible to ``solve" each component separately (for example, by assigning indices) and combine these solutions into an optimal policy.

%Much effort has been devoted recently towards developing approximations for different versions of CICS\footnote{See, for example, the survey by \cite{BC24-survey}.}; however, these techniques are generally tailored to the specifics of the information acquisition model and do not always extend to the combinatorial setting.


%\Shuchi{Shorten - no need to define the variants.} Much effort has been devoted recently towards developing approximations for variants of Pandora's Box, including the optional inspection version and the so-called partial inspection version\footnote{See, for example, the survey by \cite{BC24-survey}.}. These results are generally tailored to the specifics of the variants they study and do not extend to other models of information acquisition. Moreover, they do not always generalize to combinatorial settings. Our work aims to establish a unifying framework for addressing these issues. \Shuchi{The last statement is weak - be more precise.}



%However, the landscape changes if the algorithm has multiple modes of information acquisition available for each alternative. For example, if inspection becomes optional, that is, if the algorithm is allowed to select an alternative without observing its value, the optimal algorithm is no longer non-adaptive and the problem becomes NP-hard. Much effort has been devoted recently towards developing approximations for variants of Pandora's Box, including the optional inspection version and the so-called partial inspection version. See, for example, the survey by \cite{BC24-survey}. These results are generally tailored to the specifics of the variants they study and do not extend to other models of information acquisition. Moreover, they do not always generalize to combinatorial settings.


%\noindent \Dimitris{6. Common approach : commit to local decisions in advance.}

%By far, the most common approach taken to 

One potential strategy to address the complications of local decision making is to restrict the solution space by ``committing'' in advance to all the potential local decisions that will be made. A commitment $\pi = (\pi_1,\dotsc, \pi_n)$ specifies a mapping $\pi_i$ from the states of the MDP $\mc_i$ to some available costly action, for each alternative $i\in [n]$; a \textit{committing policy} can make global decisions about which alternative to explore but needs to respect the local restrictions of $\pi$. Equivalently, each $\pi_i$ induces a sub-process $\mc_{i}^{\pi_i}$ of $\mc_i$ that is a Markov chain; as such, efficient optimization over the optimal policy under a specific commitment is possible. This naturally motivates the question of whether there exist commitments under which the optimal policy can approximate the (unrestricted) optimal. We formalize this notion by defining the \textbf{commitment gap} for a CICS minimization\footnote{For CICS in the maximization setting, the commitment gap is defined as the ratio of utilities $\max_\pi \mathrm{OPT}(\pi)/\mathrm{OPT}\in [0,1]$.} instance as $\min_\pi \mathrm{OPT}(\pi)/\mathrm{OPT}$, where $\mathrm{OPT}$ is the cost of the optimal policy and $\mathrm{OPT}(\pi)$ is the cost of the optimal policy that is restricted by commitment $\pi$.


Much effort has been devoted recently towards developing approximations for different versions of CICS\footnote{See, for example, the survey by \cite{BC24-survey}.}; by far, the most common approach taken in the literature is to bound the commitment gap of the underlying instance \citep{BK19, AJS20, BW24, DS24}. However, these results are generally tailored to the specifics of the information acquisition model that they consider, do not always extend to the combinatorial setting and cannot be composed to study settings where alternatives of different types participate in the same instance. In order to overcome these limitations, we consider the following question:




%By far, the most common approach taken in the literature when addressing CICS problems with local decision making is to restrict the solution space by ``committing'' in advance to the costly action that will be taken at each point, for each alternative. Under a specific commitment, the algorithm is only left with the task of making global decisions; as already mentioned, this setting has been extensively studied and efficient optimization is possible in most cases. This naturally motivates the question of whether there exist commitments under which the optimal restricted policy can approximate the unrestricted optimal. We formalize this notion by introducing the \textbf{committing gap}, defined as the minimum ratio between the costs/rewards of the optimal (fully-adaptive) policy and the optimal restricted policy, under all possible commitments. We then aim to address the following question:


%\noindent \Dimitris{7. Central question.}

\begin{center}
\textit{
Is there a systematic approach for bounding the commitment gap in CICS?
}
\end{center}



%\begin{center}
%\parbox{0.98\textwidth}{
%\noindent
%A natural question is whether index-based policies can be extended to other CICS settings: can we distill the essence of the information acquisition process for each alternative into a Weitzman-style index, and build an approximation algorithm based on it? This is the question we seek to answer in this paper. }   
%\end{center}

 
%\noindent \Dimitris{8. High-level contribution - we will compare with previous work later.}

In this work, we develop a framework for addressing this question. Our first contribution is to develop a bound on the cost of the optimal (non-committing) solution through a {\bf novel cost amortization technique}. Our second contribution is to show that committing polices that satisfy certain notions of {\bf local approximation} will approximate this bound. Combined, we obtain a set of sufficient conditions to bound the commitment gap of an arbitrary CICS; importantly, these conditions apply to each alternative \textit{individually} and are \textit{impartial} to the underlying combinatorial constraint, addressing all of the previous limitations. Finally, we use our framework to obtain new or improved \textbf{approximation results} for various versions of CICS. For example, consider a variant of Pandora's Box where the value of each box is given by the sum of $k$ independent random variables, each of which needs to be separately inspected; while there are exponentially many ways to locally explore each box, we prove that the commitment gap of this problem is at most $2$. %Our framework and results extend seamlessly to combinatorial selection problems over matroid constraints as well as to combinations of different variants of information acquisition, overcoming some of the restrictions in previous lines of work.

%\Dimitris{references needed here?}



%We develop a framework for designing approximately-optimal policies for both the minimization and maximization versions of CICS. Our framework has two components. First we develop a bound on the cost of the optimal solution based on a {\bf novel cost amortization technique} that generalizes the Gittins index to Markov Decision Processes. This bound allows us to disentagle the exploration of different alternatives into individual ``local'' problems. We then show that a certain notion of {\bf local approximation} applied to each individual exploration problem can be combined via an index-based policy to obtain a global approximation guarantee. This approach is a strengthening and generalization of the ``Local Hedging'' technique developed by \cite{DS24} in the context of Pandora's Box with optional inspection.

%We instantiate our framework with new approximation results for previously studied variants of Pandora's Box as well as the new weighing scale problem described above. Our framework and results extend seamlessly to combinatorial selection problems over matroid constraints as well as to combinations of different variants of information acquisition. For example, when given a selection problem with some weighing-scale-alternatives and some optional-inspection-alternatives, our approach can effortlessly combine local approximations for each variant to obtain a combined guarantee for the whole problem.


\subsection*{A bound on the optimal (non-committing) policy.}

CICS is closely related to the Bandit Superprocess (BSP) \citep{N73}. A BSP is composed from multiple independent MDPs; at every step, the algorithm takes a step in one the MDPs, receives a reward, and the state of the underlying MDP evolves stochastically\footnote{For CICS, we further assume that the underlying MDPs are \textit{acyclic}; since the states of an MDP capture the current information we have observed about the alternative, there is a natural order of progression that cannot lead to cycles.}. In the special case where the MDPs are Markov chains, BSP reduces to the well-studied Multi-Armed Bandit (MAB) \citep{GGW11}. \cite{G79} showed that the MAB admits an optimal index-based solution for the infinite horizon setting with discounted rewards; this result was further generalized by \cite{DTW03} to the finite horizon setting (where the Markov chains have terminal states) and by \cite{GJSS19} to combinatorial selection. \cite{W80} proved a general bound for BSPs in the discounted rewards setting. In this work, we prove that the same bound continuous to hold for finite horizon processes and generalize it to arbitrary combinatorial constraints, ultimately leading to a bound for the optimal CICS policy. Moreover, our proof is constructive, more intuitive, and reveals important structural information for the underlying MDPs.

In particular, much like in the work of \cite{W80}, our approach considers a local problem $(\mc, y)$ for each MDP $\mc$ where the algorithm is presented with a deterministic outside option $y$ and at any step can either choose to take an action in $\mc$ or accept the outside option $y$ and terminate. The optimal solution to this local problem generates an optimality curve $\optf_\mc(y)$ as a function of the outside option. A primary technical contribution of our work is to convert this optimality curve into a mapping from terminal states of the MDP to ``surrogate'' costs. The surrogate costs essentially allow an algorithm to amortize the costs of actions and pay (a part of) them only when the MDP terminates. We develop a recursive ``water filling'' algorithm for cost amortization that ensures that good, i.e. low cost or high reward, terminal states are responsible for paying most of the cost share. An important property of the surrogate costs we define is that they are independent from the actions chosen by the algorithm, allowing us to compose them into a global bound for the optimal policy. In the special case of Markov chains, our water filling amortization exactly recovers the Gittins index for the MAB.


Our approach is heavily influenced by the work of \cite{KWG16} who presented an amortization viewpoint for Weitzman's index for classical Pandora's Box, as well as for its extension to Markov chains. The amortization viewpoint is also implicit in the work of \cite{S17}, who bounds the optimal cost by considering a phantom ``free information'' world. Our amortized cost shares reflect a similar argument and generalize these results to finite-horizon MDPs.


\subsection*{Local approximation conditions for bounding the commitment gap.}

In order to bound the commitment gap of CICS, we proceed to identify sufficient conditions under which a commitment $\pi = (\pi_1,\dotsc , \pi_n)$ approximates our bound on the optimal policy\footnote{Formally, we are interested in the cost/reward of the optimal committing policy that respects this commitment; from our previous discussion, this policy is immediately defined as soon as we specify the commitment.}. To ensure the generality of our framework, we wish for these conditions to be impartial to the underlying combinatorial constraint, as well as the interactions between the different MDPs: ideally, we want to define a measure of approximation that applies to each $\pi_i$ separately and can be composed into a guarantee for the entire commitment $\pi$.




Similarly to how we established our bound on the optimal policy, we consider the local problems $(\mc_i,y)$ for each MDP $\mc_i$. \cite{W80} showed that when each MDP $\mc_i$ admits a commitment $\pi_i$ that is optimal in the local problem under all values of $y$, then the commitment gap achieved by $\pi = (\pi_1,\dotsc , \pi_n)$ is $1$. In other words, unambiguous optimality in the local problems composes into optimality for the global setting. %However, in the absence of such a strong local optimality condition, the (overall) optimal policy may take actions that are suboptimal for the MDP they're taken in. 
However, the reverse doesn't hold: in~\Cref{app:example}, we illustrate an example of CICS where the commitment gap is $1$, and yet the optimal algorithm commits to a local policy that is strictly suboptimal for all values of $y$ in the local problem. One reasonable approach to extend Whittle's condition beyond unambiguous optimality is to try to find commitments that are approximately optimal for the local problems; however, even if each commitment $\pi_i$ is an $\alpha$-approximation for the local game $(\mc_i,y)$, the commitment gap under the composition $\pi=(\pi_1,\dotsc , \pi_n)$ might be $\alpha^n$ - an exponential increase!



%However, this does not work. Consider, for example, a minimization MDP $\mc$ with two $0$-cost actions: the first action leads to a deterministic value of $1$, and the second uniformly leads to a stochastic value of $0$ or $1$. Committing to each of these actions leads to an expected cost of $\min(y,1)$ and $1/2\cdot \min(y,1)$ respectively; the deterministic action achieves a $2$-approximation for all local problems $(\mc, y)$. Now consider a single-selection CICS with $n$ copies of the above MDP. If we commit to the deterministic action in each MDP, our cost is deterministically $1$, whereas taking the stochastic action in each costs us $1/2^n$ -- an exponential gap!


\cite{DS24} describe how to fix this problem in the context of Pandora's Box with optional inspection and define a local approximation as follows. Let $\optf_{\mc_i}(\cdot)$ and $\optf_{\pi_i}(\cdot)$ denote the optimality curves of the MDP $\mc_i$ and the committing policy $\pi_i$ for $\mc_i$, respectively, in the local problem $(\mc_i, y)$. The {\em local approximation} factor for minimization achieved by $\pi_i$ for the MDP $\mc_i$ is $\alpha\geq 1$ if we have 
\begin{equation}
\label{eq:local}
\optf_{\pi_i}(\alpha y)\le \alpha\optf_{\mc_i}(y) \,\, \forall y\in \real.
\end{equation}
For maximization, we likewise require $\optf_{\pi_i}(\frac y\alpha)\ge \frac 1\alpha \optf_{\mc_i}(y)$ for all $y$.
It then holds that if each $\pi_i$ achieves an $\alpha$-local approximation for the MDP $\mc_i$, then commitment gap for $\pi=(\pi_1,\dotsc,\pi_n)$ is at most $\alpha$.\footnote{Observe that Equation~\eqref{eq:local} is stronger than simply requiring the commitment policy to be approximately optimal for the local game $(\mc, y)$ at every possible outside option $y$ (in other words, $\optf_\pi(y)\le \alpha\optf_\mc(y)$).} For $\alpha=1$, local approximation precisely recovers Whittle's condition.

In this work, we strengthen this composition result and show that it holds for general CICS. Informally speaking, local approximation is equivalent to establishing second order stochastic dominance between the surrogate costs of the MDP and the commitment-induced Markov chain. We also explore the stronger condition of first order stochastic dominance between surrogate costs, that we call {\em pointwise approximation}, which can be easier to establish in some settings. Finally, we observe that the local approximation condition can be challenging to satisfy in some settings. For example, if $\optf_\mc$ is near-linear, then Equation~\eqref{eq:local} is essentially equivalent to requiring $\optf_\mc=\optf_\pi$. We therefore explore a weakening of the condition by allowing for additive deviations from \eqref{eq:local}. We call this property {\em semilocal approximation}, and show that it leads to improved approximation bounds for some settings. These three characterizations allow us to bound the commitment gap of a CICS and design approximate-optimal commitment policies.


\subsection*{Contributions}
We present our amortization framework and our bound on the optimal (non-committing) policy in~\Cref{sec:amortization}. Our local approximation conditions and the corresponding composition results are presented in~\Cref{sec:local_approx}. A detailed discussion of related work can be found in \Cref{sec:related}. In the remaining sections, we demonstrate how our framework implies new or improved bounds on the commitment gap for various extensions of Pandora's Box.
\begin{itemize}
    \item {\bf PB with Partial Inspection} (\cref{sec:pvo}). In addition to opening the box, the algorithm can choose to ``peek'' into it at a cheaper cost and learn its value; boxes must still be opened before being selected. We prove a bound of $\sqrt{2}$ on the committing gap through local approximation.
    
    \item {\bf Weighing Scale Problem} (\cref{sec:ws}). Rather than opening the box that contains alternative $X_i$, the algorithm can only use a costly scale to weigh it against a threshold $t$ of its choosing and learn whether $X_i\geq t$ or not. We obtain a logarithmic bound (in key parameters of the problem) on the commitment gap through pointwise approximation.
    
    \item {\bf Additive PB} (\cref{sec:additive_pb}). The value of each box is given by the sum of independent random variables; each component must be separately inspected at a cost and the box can be selected only after all components have been inspected\footnote{This is a special case of the notoriously challenging Pandora's Shortest Path problem over parallel path graphs}. We prove a bound of $2$ on the committing gap through pointwise approximation.
    
    \item {\bf PB with Optional Inspection} (\cref{sec:gvo}). The value of each box can be selected without being inspected. We consider the maximization version of this problem. We show that the best possible bound on the commitment gap achieved through local approximation is $0.5$; on the other hand, semilocal approximation allows us to obtain a bound of $0.582$.
    
\end{itemize}

All of our results apply to any set of combinatorial constraints. The first three extensions are considered in the minimization setting and have not been previously studied. With the the exception of additive PB, all our bounds on the commitment gaps are constructive and the committing policies that achieve them can be efficiently computed. As such, they directly imply approximation algorithms for any set of feasibility constraints that admit a frugal algorithm, as defined in~\citep{S17}; the exception is PB with optional inspection, as semilocal approximation can only be composed up to matroid constraints. The maximization version of PB with optional inspection has been extensively studied in the literature; however, all previous results that overcome the $0.5$ barrier either apply to the single-selection setting or are non-constructive. In contrast, we provide the first policy for the matroid setting that can be efficiently computed and achieves an approximation guarantee that is strictly better than $0.5$.



\newpage

%\subsection*{Connections to multi-armed bandits and bandit superprocesses.}

%\noindent \Dimitris{9. Connection to MAB - definition and related results.}

%In the absence of local decision making (or equivalently, when restricted on a specific commitment), selection problems with costly information correspond to the well-studied Markovian multi-armed bandit (MAB) \citep{GGW11}. In a MAB, the algorithm is given $n$ Markovian ``arms''; at every step the algorithm can pull any one of the arms and receive a reward; the state of the pulled arm then evolves according to the underlying Markov process. \citet{G79} showed that an index-based policy is optimal for this problem. MAB is usually studied in an infinite horizon setting with discounted or averaged reward. \cite{DTW03} extended this approach to the finite horizon setting (where Markov chains have terminal states) and \cite{GJSS19} further extended it to combinatorial selection. Weitzman's index-policy for Pandora's Box is a special case of these results.

%Selection problems with costly information are closely related to a class of sequential decision-making problems called bandit superprocesses, which generalize Markovian multi-armed bandits (MAB) \citep{GGW11}. In an MAB, the algorithm is given $n$ Markovian ``arms''; at every step the algorithm can pull any one of the arms and receive a reward; the state of the pulled arm then evolves according to the underlying Markov process. \citet{G79} showed that an index-based policy is optimal for this problem. MAB is usually studied in an infinite horizon setting with discounted or averaged reward. \cite{DTW03} extended this approach to the finite horizon setting (where Markov chains have terminal states) and \cite{GJSS19} further extended it to combinatorial selection. Weitzman's index-policy for Pandora's Box is a special case of these results.

%\noindent \Dimitris{10. Definition of BSP and related results.}

%In their full generality, selection problems with costly information correspond to the much more challenging bandit superprocesses (BSP) \citep{N73}, of which MAB are a special case. In a general BSP, the $n$ arms are Markov Decision Processes (MDPs) comprising multiple possible actions with different costs/rewards. While it is possible to treat the superprocess as a single large MDP, the exponential size of this MDP makes this approach computationally infeasible, and it is desirable to consider algorithms that ``solve'' each component process separately and combine the solutions together, much like the index-based algorithms for a MAB. However, the optimal solution to a BSP does not share the same structural properties and it is in general NP-hard to compute it, with approximation results known only for specific cases. In particular, \cite{W80} showed that under very strong local conditions on the MDPs, the optimal policy for the BSP admits the same index-based solution as the MAB.


%In a general bandit superprocess, the $n$ arms are Markov Decision Processes (MDPs) comprising multiple possible actions with different costs/rewards. While it is possible to treat the superprocess as a single large MDP, the exponential size of this MDP makes this approach computationally infeasible, and it is desirable to consider algorithms that ``solve'' each component process separately and combine the solutions together. \cite{W80} showed that certain bandit superprocesses admit simple index-policies just like the MAB special case. In particular, when each MDP in the superprocess admits an unambiguously optimal static policy, these policies can be composed to obtain a globally optimal policy through appropriately defined indices. However, in the absence of such a strong local optimality condition, the globally optimal policy may take actions that are suboptimal for the MDP they're taken in. \textcolor{blue}{We illustrate such an example in~\Cref{app:example}.}

%\noindent \Dimitris{11. Concretely state how our work ties in to the above.}

%Our framework models each of the $n$ alternatives as a MDP and the CICS instance is defined as the corresponding (combinatorial) BSP. Each state of these MDPs captures the information that we currently have on the alternative, and each costly action from that state describes a different exploration mode; depending on the outcome, we transition to a new state. Accepting an alternative corresponds to the MDP reaching a sink state. For these reasons, we only need to consider MDPs that have a DAG-like structure, as each state captures a different level of progression. In this context, a committing policy specifies a single action for each state of the MDPs, transforming the BSP into a MAB. The committing gap is then defined as the ratio between the costs/rewards of the optimal solution for the BSP and the MAB.


%\subsection*{A bound on the optimal policy through cost amortization.}


%\noindent \Dimitris{12. Describe the amortization.}

%Much like in the work of \cite{W80}, our approach considers a local problem $(\mc, y)$ for each MDP $\mc$ where the algorithm is presented with a deterministic outside option $y$ and at any step can either choose to take an action in $\mc$ or accept the outside option $y$ and terminate. The optimal solution to this local problem generates an optimality curve $\optf_\mc(y)$ as a function of the outside option. A primary technical contribution of our work is to convert this optimality curve into a mapping from terminal states of the MDP to ``surrogate'' costs (Section~\ref{sec:amortization}). The surrogate costs essentially allow an algorithm to amortize the costs of actions and pay (a part of) them only when the MDP terminates. We develop a recursive ``water filling'' algorithm for cost amortization that ensures that good, i.e. low cost or high reward, terminal states are responsible for paying most of the cost share. The overall index of the MDP is then defined to be the cost of the best-case scenario -- the lowest possible surrogate cost that is instantiated. In the special case of Markov chains, our water filling amortization exactly recovers the Gittins index.


%Much like Whittle's work, our approach considers a local problem $(\mc, y)$ for each MDP $\mc$ where the algorithm is presented with a deterministic outside option $y$ and at any step can either choose to take an action in $\mc$ or accept the outside option $y$. The optimal solution to this local problem generates an optimality curve $\optf_\mc(y)$ as a function of the outside option. A primary technical contribution of our work is to convert this optimality curve into a mapping from terminal states of the MDP to ``surrogate'' costs (Section~\ref{sec:amortization}). The surrogate costs essentially allow an algorithm to amortize the costs of actions and pay (a part of) them only when the MDP terminates. We develop a recursive ``water filling'' algorithm for cost amortization that ensures that good, i.e. low cost or high reward, terminal states are responsible for paying most of the cost share. The overall index of the MDP is then defined to be the cost of the best-case scenario -- the lowest possible surrogate cost that is instantiated. In the special case of Markov chains, our water filling amortization exactly recovers the Gittins index.




%\noindent \Dimitris{13. Highlight action independence.}

%A key property of the surrogate costs we define is their {\em independence from the actions chosen} by the algorithm in the MDP (Lemma~\ref{lem:mdp-wf-char-new} in Section~\ref{sec:amortization}). The corresponding indices can therefore be defined and computed independently of the algorithm's stochastic trajectory, much like in Gittins or Weitzman's setting. This allows us to compose these costs and obtain a global bound on the value of the optimal solution. However, the independence comes at a loss -- the surrogate costs provide a bound that is not exact for general MDPs (in contrast to Whittle's results, for example). 


%A key property of the surrogate costs we define is their {\em independence from the actions chosen} by the algorithm in the MDP (Lemma~\ref{lem:mdp-wf-char-new} in Section~\ref{sec:amortization}). The corresponding indices can therefore be defined and computed independently of the algorithm's stochastic trajectory, much like in Gittins or Weitzman's setting. This allows us to compose these costs and obtain a global bound on the value of the optimal solution. However, the independence comes at a loss -- the surrogate costs provide a bound that is not exact for general MDPs (in contrast to Whittle's results, for example). 



%\noindent \Dimitris{14. Describe how it relates to and extends previous work.}

%Our approach is heavily influenced by the work of \cite{KWG16} who presented an amortization viewpoint for Weitzman's index for classical Pandora's Box, as well as for its extension to Markov chains. The amortization viewpoint is also implicit in the work of \cite{S17}, who bounds the optimal cost by considering a phantom ``free information'' world. Our amortized cost shares reflect a similar argument. We emphasize that while bounds on the optimal solution's value have been established previously for the single-selection CICS \citep{BS13}, a general bound for the combinatorial setting was not known previously; our bound applies to \textit{any} feasibility constraint and \textit{any} bandit superprocess where the constituent MDPs have a DAG-like structure. Importantly, the amortization framework that we use to derive these bounds provides valuable intuition on how the amortized costs are instantiated that in turn helps us develop the conditions for bounding the committing gap. 


%Our approach is heavily influenced by the work of \cite{KWG16} who presented an amortization viewpoint for Weitzman's index for classical Pandora's Box, as well as for its extension to Markov chains. The amortization viewpoint is also implicit in the work of \cite{S17}, who bounds the optimal cost by considering a phantom ``free information'' world. Our amortized cost shares reflect a similar argument. We emphasize that while bounds on the optimal solution's value have been established previously for the single-selection CICS in special cases, a general bound was not known previously. Our bound applies to any feasibility constraint over any bandit superprocess where the constituent MDPs have a DAG-like structure.



%\subsection*{Bounding the committing gap through local conditions.}


%\noindent \Dimitris{15. General approach + Whittle's result + reverse doesn't hold.}

%From our previous discussion, a sufficient condition to bound the committing gap of a CICS is to determine a committing policy that approximates our bound on the optimal policy. \cite{W80} showed that when each MDP in the superprocess admits an unambiguously optimal committing policy for the local game, then the committing gap of the superprocess is $1$. However, in the absence of such a strong local optimality condition, the (overall) optimal policy may take actions that are suboptimal for the MDP they're taken in. In~\Cref{app:example}, we illustrate an example of a CICS where the committing gap is $1$, and yet the optimal policy commits to an action that is universally suboptimal for the local game.

%One reasonable approach to extend Whittle's approach is to try to find a committing policy for each MDP that is approximately optimal for the local game. However, this does not work. Consider, for example, a minimization MDP $\mc$ with two $0$-cost actions. The first action leads to a deterministic value of $1$, and the second leads to a stochastic value of $0$ or $1$ with probability $1/2$ each. Then, the first action provides a $2$-approximation for the local game $(\mc, y)$: its expected cost is $\min(y,1)$ whereas the optimal cost of the local game is half of that quantity, achieved by taking the stochastic option. Now consider a single-selection superprocess with $n$ copies of the above MDP. If we commit to the deterministic action in each MDP, our cost is deterministically $1$, whereas taking the stochastic action in each costs us $1/2^n$ -- an exponential gap!



%Next we consider approximations to the CICS through a class of algorithms called ``commitment policies''. A commitment policy for an instance of the CICS specifies a (random) action for the algorithm to take at any state of any component MDP.\footnote{E.g., in the weighing scale problem, for each $X_i$, we may specify targets $t^i_1, t^i_{11}, t^i_{12},$ etc. such that $X_i$ is first compared against $t^i_1$, and then against $t^i_{11}$ or $t^i_{12}$ depending on whether the first comparison was True or False, and so on and so forth.} The commitment for each alternative depends on its own state and not on the states of other processes. This turns each MDP into a (suboptimal) Markov chain. Armed with these commitments, the algorithm faces a combinatorial MAB which, based on the prior discussion, we know how to solve.

%\noindent \Dimitris{16. Normal approximation is not sufficient.}

%Given the characterization of the optimal cost in terms of properties of the local games $(\mc, y)$ defined above, one reasonable approach is to try to find a committing policy for each MDP that is approximately optimal for the local game. However, this does not work. Consider, for example, a minimization MDP $\mc$ with two $0$-cost actions. The first action leads to a deterministic value of $1$, and the second leads to a stochastic value of $0$ or $1$ with probability $1/2$ each. Then, the first action provides a $2$-approximation for the local game $(\mc, y)$: its expected cost is $\min(y,1)$ whereas the optimal cost of the local game is half of that quantity, achieved by taking the stochastic option. Now consider a single-selection superprocess with $n$ copies of the above MDP. If we commit to the deterministic action in each MDP, our cost is deterministically $1$, whereas taking the stochastic action in each costs us $1/2^n$ -- an exponential gap!


%Given the characterization of the optimal cost in terms of properties of the local games $(\mc, y)$ defined above, one reasonable approach is to try to find a commitment policy for each MDP that is approximately optimal for the local game. However, this does not work. Consider, for example, a minimization MDP $\mc$ with two actions. The first action leads to a deterministic value of $1$, and the second leads to a stochastic value of $0$ or $1$ with probability $1/2$ each. Then, the first action provides a $2$-approximation for the local game $(\mc, y)$: its expected cost is $\min(y,1)$ whereas the optimal cost of the local game is half of that quantity, achieved by taking the stochastic option. Now consider a single-selection superprocess with $n$ copies of the above MDP. If we commit to the deterministic action in each MDP, our cost is deterministically $1$, whereas taking the stochastic action in each costs us $1/2^n$ -- an exponential gap!

%\noindent \Dimitris{17. Local approximation condition.}


%\cite{DS24} describe how to fix this problem in the context of Pandora's Box with optional inspection and define a local approximation as follows. Let $\optf_\mc(\cdot)$ and $\optf_{\pi}(\cdot)$ denote the optimality curves of the MDP $\mc$ and the committing policy $\pi$ for $\mc$, respectively, in the local game $(\mc, y)$. The {\em local approximation} factor for minimization achieved by $\pi$ for the MDP $\mc$ is $\alpha\geq 1$ if we have 
%\begin{equation}
%\label{eq:local}
%\optf_\pi(\alpha y)\le \alpha\optf_\mc(y) \,\, \forall y\in \real.
%\end{equation}
%For maximization, we likewise require $\optf_\pi(\frac y\alpha)\ge \frac 1\alpha \optf_\mc(y)$ for all $y$.
%It then holds that any commitment policy that achieves an $\alpha$-local approximation for each constituent MDP achieves a committing gap of $\alpha$.\footnote{Observe that Equation~\eqref{eq:local} is stronger than simply requiring the commitment policy to be approximately optimal for the local game $(\mc, y)$ at every possible outside option $y$ (in other words, $\optf_\pi(y)\le \alpha\optf_\mc(y)$).}  In Section~\ref{sec:local_approx} we strengthen this composition result holds and show that it holds for general CICS. 

%\noindent \Dimitris{18. Pointwise approximation condition.}

%Informally speaking, local approximation is equivalent to establishing second order stochastic dominance between the surrogate costs of the MDP and the committing policy. We also explore the stronger condition of first order stochastic dominance between surrogate costs, that we call {\em pointwise approximation}, which can be easier to establish in some settings. These characterizations allows us to design commitment policies that achieve a good committing gap.


%\noindent \Dimitris{19. Smilocal approximation condition.}

%In some settings, the local approximation condition can be challenging to satisfy. For example, if $\optf_\mc$ is near-linear, then Equation~\eqref{eq:local} is essentially equivalent to requiring $\optf_\mc=\optf_\pi$.\footnote{That is, $\pi$ must be unambiguously optimal for $\mc$; and no suboptimal policy can provide any local approximation.} We therefore explore a weakening of the condition by allowing for additive deviations from \eqref{eq:local}. We call this property {\em Semilocal Approximation}, and show that it leads to improved approximation bounds for some settings (Section~\ref{sec:gvo:composition}).


%\noindent \Dimitris{20. Recap and observations.}

%Note that all three conditions (local, pointwise and semilocal approximation) apply to each alternative separately, and yet they suffice to bound the adaptivity gap of the entire CICS. Furthermore, due to the generality of these conditions, our framework directly captures settings where each MDP corresponds to different models of information acquisition; we note that previous approaches where tailored to specific information models and were thus unable to obtain similar results.





==> new_introduction_2.tex <==
\section{Introduction - Ziv's Version}\label{sec:intro}


%Consider a biotechnology company investing in multiple drug discovery projects. Each individual project can involve a multitude of decisions with uncertain outcomes. Typically, very few projects will make it to trials and FDA approval, at which point they can begin to yield rewards for the company. The company needs to determine how to distribute resources across these projects without knowing upfront which one will succeed and to what extent. Similarly, many decision making problems call for upfront investment in information acquisition before optimizing over multiple options. Other examples include an oil company's search for a good drilling site; a construction company exploring different design ideas for a project; a manufacturer performing market research before determining which products to make and in what quantity, etc.

The foundational model of stochastic optimization under costly information is known as the Pandora's Box problem, introduced by \cite{W79}. In this classical example, the decision maker is presented with a set of random alternatives that are independently realized from known distributions. Each alternative is hidden inside a closed box and the algorithm can observe the value of the alternative by opening, a.k.a. ``inspecting'', the corresponding box at a cost. The goal is to select a single inspected alternative while maximizing the value of the selection minus the total cost of opening boxes. Since its introduction, various extensions of Pandora's Box have been introduced in order to account for more interesting and complex information acquisition models. The most studied variant is optional inspection, where a box can be blindly selected without being inspected. Beyond that, one could consider boxes that can only be accessed via threshold testing queries, boxes that allow for partial observations of their values and even boxes that require multiple stages of inspection. Additionally, each of these extensions can be considered in the minimization setting, as well as the combinatorial setting, where rather than accepting a single box, the algorithm must accept a (feasible) set of boxes.



Recently, there has been an increasing interest for the extensions of Pandora's Box \citep{GMS08, OW15, KWG16, S17, D18, BK19, EHLM19, BFLL20, AJS20, GJSS19, FLL22, BC22,BEFF23, BW24, DS24}. We refer the reader to the survey of \cite{BC24-survey} for some of the latest developments. One major limitation of these works is that they separately address each extension that they consider; there is a lack of a general and systematic approach for existing and new variants of Pandora's Box. For example, although previous results separately address the optional and partial inspection variants, it is not clear how one would handle a setting that consists of both optional and partial inspection boxes. Furthermore, not all of these results extend to the combinatorial setting.


We initiate the systematic study of these variants by introducing a family of problems that we call {\em Costly Information Combinatorial Selection} (henceforth, CICS). In CICS, our goal is to select a subset of $n$ alternatives with stochastic values under some feasibility constraint. We can obtain information about the value of any individual alternative through a sequence of costly actions tailored to that alternative. We model this information acquisition process for alternative $i$ as a finite-horizon Markov decision process (henceforth, MDP) $\mc_i$. The MDPs $\mc_1, \cdots, \mc_n$ are independent: the states in $\mc_i$ correspond only to the information we have learned thus far about alternative $i$ and the costly actions available in $\mc_i$ only reveal further information about $i$. At any point of time, the policy can terminate by accepting any feasible subset of alternatives for which the underlying MDPs have reached a terminal (sink) state. In the minimization version of the problem our objective is to minimize the total value of the chosen alternatives plus the cost of information acquisition. In the maximization version we maximize the total value of the chosen subset minus the cost of information acquisition. 

The algorithmic challenge of CICS stems from two different levels of decision making that influence each other: at each step, a policy (a.k.a. an algorithm) needs to select which out of the $n$ alternatives to explore (global decision making); as well as which alternative-specific costly action to take in order to explore it (local decision making). In general, these decisions are made adaptively, based on the information that was obtained in previous steps. While it is possible to accommodate these challenges by treating all the alternatives as a single MDP and apply a standard solver, this approach would lead to an exponential blow-up in the state space and is computationally infeasible. Instead, it is desirable to design policies that separately ``solve" each component MDP and then compose these solutions into an optimal policy.

Remarkably, this is precisely what happens when local decision making isn't required; this corresponds to the special case where each alternative can be explored in a unique way at any point of time, and the MDP $\mc_i$ is simply a Markov chain. \cite{G79} showed that in the infinite-horizon discounted rewards setting, the optimal policy admits an astonishingly simple structure: at each step, (i) an \textit{index} is individually computed for each Markov chain, and (ii) the Markov chain of highest index is advanced. This index-based optimality structure has been subsequently generalized to the finite-horizon minimization setting where Markov chains have terminal states \citep{DTW03} as well as to any combinatorial setting that admits
a greedy-style (a.k.a. frugal) approximation algorithm \citep{S17,GJSS19}. We note that Weitzman's optimal policy for the (standard) Pandora's Box problem is a special case of these results; each box is assigned an index that depends only on it's distribution and cost, and boxes are inspected in decreasing index order.

However, most of the Pandora's Box variants we discussed include some level of local decision making. In general, when the algorithm has multiple modes of information acquisition available for each alternative, the landscape changes significantly.  For example, in the optional inspection variant of Pandora's Box, it is known that the optimal policy no longer inspects the boxes in a fixed order and computing the optimal solution is NP-hard \citep{FLL22}. In general, the optimal policy for CICS no longer exhibits the same structural properties as in the special case of Markov chains, and it is not possible to ``solve" each component separately (for example, by assigning indices) and combine these solutions into an optimal policy.

By far, the most common approach taken in the literature to address these complications is to restrict the solution space by ``committing'' in advance to all the potential local decisions that will be made\citep{BK19, AJS20, BW24, DS24}. Formally, a commitment $\pi = (\pi_1,\dotsc, \pi_n)$ specifies a mapping $\pi_i$ from the states of the MDP $\mc_i$ to some available costly action, for each alternative $i\in [n]$; a \textit{committing policy} can make global decisions about which alternative to explore but needs to respect the local restrictions of $\pi$. Equivalently, each $\pi_i$ induces a sub-process $\mc_{i}^{\pi_i}$ of $\mc_i$ that is a Markov chain; as such, efficient optimization over the optimal policy under a specific commitment is possible. This naturally motivates the question of whether there exist commitments under which the optimal policy can approximate the (unrestricted) optimal. We formalize this notion by defining the \textbf{commitment gap} for a CICS minimization\footnote{For CICS in the maximization setting, the commitment gap is defined as the ratio of utilities $\max_\pi \mathrm{OPT}(\pi)/\mathrm{OPT}\in [0,1]$.} instance as $\min_\pi \mathrm{OPT}(\pi)/\mathrm{OPT}$, where $\mathrm{OPT}$ is the cost of the optimal policy and $\mathrm{OPT}(\pi)$ is the cost of the optimal policy that is restricted by commitment $\pi$.

In order to design a general framework for studying the different variants of Pandora's Box, we develop a set of sufficient conditions for bounding the commitment gap of CICS. To ensure the generality of our framework, we wish for these conditions to be impartial to the underlying combinatorial constraint, as well as the interactions between the different MDPs: ideally, we want to define a measure of approximation that applies to each $\pi_i$ separately and can be composed into a guarantee for the entire commitment $\pi$. Our first contribution is to develop a bound on the cost of the optimal (non-committing) solution through a {\bf novel cost amortization technique}. Our second contribution is to show that committing polices that satisfy certain notions of {\bf local approximation} with the desired properties will approximate this bound. Finally, we use our framework to obtain new or improved \textbf{approximation results} for various versions of CICS. For example, consider a variant of Pandora's Box where the value of each box is given by the sum of $k$ independent random variables, each of which needs to be separately inspected; while there are exponentially many ways to locally explore each box, we prove that the commitment gap of this problem is at most $2$.



\subsection*{A bound on the optimal (non-committing) policy.}

A Bandit Superprocess (BSP), introduced by \cite{N73}, is composed from multiple independent MDPs; at every step, the algorithm takes a step in one the MDPs, receives a reward, and the state of the underlying MDP evolves stochastically. In the special case where the MDPs are Markov chains, BSP reduces to the well-studied Multi-Armed Bandit (MAB) \citep{GGW11}. Naturally, CICS is closely related to BSP\footnote{For CICS, we further assume that the underlying MDPs are \textit{acyclic}; since the states of an MDP capture the current information we have observed about the alternative, there is a natural order of progression that cannot lead to cycles.}. \cite{W80} proved a general bound for the optimal policy of a BSP in the discounted rewards setting. In this work, we prove that the same bound continuous to hold for finite horizon processes (both for minimization and maximization) and generalize it to arbitrary combinatorial constraints, ultimately leading to a bound for the optimal CICS policy. Moreover, our proof is constructive, more intuitive, and reveals important structural information for the underlying MDPs.

In particular, much like in the work of \cite{W80}, our approach considers a local problem $(\mc, y)$ for each MDP $\mc$ where the algorithm is presented with a deterministic outside option $y$ and at any step can either choose to take an action in $\mc$ or accept the outside option $y$ and terminate. The optimal solution to this local problem generates an optimality curve $\optf_\mc(y)$ as a function of the outside option. A primary technical contribution of our work is to convert this optimality curve into a mapping from terminal states of the MDP to ``surrogate'' costs. The surrogate costs essentially allow an algorithm to amortize the costs of actions and pay (a part of) them only when the MDP terminates. We develop a recursive ``water filling'' algorithm for cost amortization that ensures that good, i.e. low cost or high reward, terminal states are responsible for paying most of the cost share. An important property of the surrogate costs we define is that they are independent from the actions chosen by the algorithm, allowing us to compose them into a global bound for the optimal policy. In the special case of Markov chains, our water filling amortization exactly recovers the Gittins index for the MAB.

Our approach is heavily influenced by the work of \cite{KWG16} who presented an amortization viewpoint for Weitzman's index for classical Pandora's Box, as well as for its extension to Markov chains. The amortization viewpoint is also implicit in the work of \cite{S17}, who bounds the optimal cost by considering a phantom ``free information'' world. Our amortized cost shares reflect a similar argument and generalize these results to finite-horizon MDPs.


\subsection*{Local approximation conditions for bounding the commitment gap.}

In order to bound the commitment gap of CICS, we proceed to identify sufficient conditions under which a commitment $\pi = (\pi_1,\dotsc , \pi_n)$ approximates our bound on the optimal policy\footnote{Formally, we are interested in the cost/reward of the optimal committing policy that respects this commitment; from our previous discussion, this policy is immediately defined as soon as we specify the commitment.} As already mentioned, these conditions should be impartial to the underlying combinatorial constraint and the interactions between different MDPs; ideally, we want to define a measure of approximation that applies to each $\pi_i$ separately and can be composed into a guarantee for the entire commitment $\pi$.

Similarly to how we established our bound on the optimal policy, we consider the local problems $(\mc_i,y)$ for each MDP $\mc_i$. \cite{W80} showed that when each MDP $\mc_i$ admits a commitment $\pi_i$ that is optimal in the local problem under all values of $y$, then the commitment gap achieved by $\pi = (\pi_1,\dotsc , \pi_n)$ is $1$. In other words, unambiguous optimality in the local problems composes into optimality for the global setting. %However, in the absence of such a strong local optimality condition, the (overall) optimal policy may take actions that are suboptimal for the MDP they're taken in. 
However, the reverse doesn't hold: in~\Cref{app:example}, we illustrate an example of CICS where the commitment gap is $1$, and yet the optimal algorithm commits to a local policy that is strictly suboptimal for all values of $y$ in the local problem. One reasonable approach to extend Whittle's condition beyond unambiguous optimality is to try to find commitments that are approximately optimal for the local problems; however, even if each commitment $\pi_i$ is an $\alpha$-approximation for the local game $(\mc_i,y)$, the commitment gap under the composition $\pi=(\pi_1,\dotsc , \pi_n)$ might be $\alpha^n$ - an exponential increase!


%One reasonable approach to extend Whittle's condition beyond unambiguous optimality is to try to find commitments that are approximately optimal for the local problems. However, this does not work. Consider, for example, a minimization MDP $\mc$ with two $0$-cost actions: the first action leads to a deterministic value of $1$, and the second uniformly leads to a stochastic value of $0$ or $1$. Committing to each of these actions leads to an expected cost of $\min(y,1)$ and $1/2\cdot \min(y,1)$ respectively; the deterministic action achieves a $2$-approximation for all local problems $(\mc, y)$. Now consider a single-selection CICS with $n$ copies of the above MDP. If we commit to the deterministic action in each MDP, our cost is deterministically $1$, whereas taking the stochastic action in each costs us $1/2^n$ -- an exponential gap!


\cite{DS24} describe how to fix this problem in the context of Pandora's Box with optional inspection and define a local approximation as follows. Let $\optf_{\mc_i}(\cdot)$ and $\optf_{\pi_i}(\cdot)$ denote the optimality curves of the MDP $\mc_i$ and the committing policy $\pi_i$ for $\mc_i$, respectively, in the local problem $(\mc_i, y)$. The {\em local approximation} factor for minimization achieved by $\pi_i$ for the MDP $\mc_i$ is $\alpha\geq 1$ if we have 
\begin{equation}
\label{eq:local}
\optf_{\pi_i}(\alpha y)\le \alpha\optf_{\mc_i}(y) \,\, \forall y\in \real.
\end{equation}
For maximization, we likewise require $\optf_{\pi_i}(\frac y\alpha)\ge \frac 1\alpha \optf_{\mc_i}(y)$ for all $y$.
It then holds that if each $\pi_i$ achieves an $\alpha$-local approximation for the MDP $\mc_i$, then commitment gap for $\pi=(\pi_1,\dotsc,\pi_n)$ is at most $\alpha$.\footnote{Observe that Equation~\eqref{eq:local} is stronger than simply requiring the commitment policy to be approximately optimal for the local game $(\mc, y)$ at every possible outside option $y$ (in other words, $\optf_\pi(y)\le \alpha\optf_\mc(y)$).} For $\alpha=1$, local approximation precisely recovers Whittle's condition.

In this work, we strengthen this composition result and show that it holds for general CICS. Informally speaking, local approximation is equivalent to establishing second order stochastic dominance between the surrogate costs of the MDP and the commitment-induced Markov chain. We also explore the stronger condition of first order stochastic dominance between surrogate costs, that we call {\em pointwise approximation}, which can be easier to establish in some settings. Finally, we observe that the local approximation condition can be challenging to satisfy in some settings. For example, if $\optf_\mc$ is near-linear, then Equation~\eqref{eq:local} is essentially equivalent to requiring $\optf_\mc=\optf_\pi$. We therefore explore a weakening of the condition by allowing for additive deviations from \eqref{eq:local}. We call this property {\em semilocal approximation}, and show that it leads to improved approximation bounds for some settings. These three characterizations allow us to bound the commitment gap of a CICS and design approximate-optimal commitment policies.




\subsection*{Contributions}
We present our amortization framework and our bound on the optimal (non-committing) policy in~\Cref{sec:amortization}. Our local approximation conditions and the corresponding composition results are presented in~\Cref{sec:local_approx}. A detailed discussion of related work can be found in \Cref{sec:related}. In the remaining sections, we demonstrate how our framework implies new or improved bounds on the commitment gap for various extensions of Pandora's Box.
\begin{itemize}
    \item {\bf PB with Partial Inspection} (\cref{sec:pvo}). In addition to opening the box, the algorithm can choose to ``peek'' into it at a cheaper cost and learn its value; boxes must still be opened before being selected. We prove a bound of $\sqrt{2}$ on the committing gap through local approximation.
    
    \item {\bf Weighing Scale Problem} (\cref{sec:ws}). Rather than opening the box that contains alternative $X_i$, the algorithm can only use a costly scale to weigh it against a threshold $t$ of its choosing and learn whether $X_i\geq t$ or not. We obtain a logarithmic bound (in key parameters of the problem) on the commitment gap through pointwise approximation.
    
    \item {\bf Additive PB} (\cref{sec:additive_pb}). The value of each box is given by the sum of independent random variables; each component must be separately inspected at a cost and the box can be selected only after all components have been inspected\footnote{This is a special case of the notoriously challenging Pandora's Shortest Path problem over parallel path graphs}. We prove a bound of $2$ on the committing gap through pointwise approximation.
    
    \item {\bf PB with Optional Inspection} (\cref{sec:gvo}). The value of each box can be selected without being inspected. We consider the maximization version of this problem. We show that the best possible bound on the commitment gap achieved through local approximation is $0.5$; on the other hand, semilocal approximation allows us to obtain a bound of $0.582$.
    
\end{itemize}

All of our results apply to any set of combinatorial constraints. The first three extensions are considered in the minimization setting and have not been previously studied. With the the exception of additive PB, all our bounds on the commitment gaps are constructive and the committing policies that achieve them can be efficiently computed. As such, they directly imply approximation algorithms for any set of feasibility constraints that admit a frugal algorithm, as defined in~\citep{S17}; the exception is PB with optional inspection, as semilocal approximation can only be composed up to matroid constraints. The maximization version of PB with optional inspection has been extensively studied in the literature; however, all previous results that overcome the $0.5$ barrier either apply to the single-selection setting or are non-constructive. In contrast, we provide the first policy for the matroid setting that can be efficiently computed and achieves an approximation guarantee that is strictly better than $0.5$. 
\newpage

\begin{comment}
\Ziv{
The need for CICS:
\* Real-life motivating example
\* How do we model this? Pandora's box variants
\** Simple
\** Optional inspection
\** Multiple stages
\** Multiple stages with skips allowed
\** Multiple parts with flexible order
\** Indirect observation through queries (weighing scale re-stated as a PB variant for consistency)
\** Add a figure if time
\* Lots of interest in Pandora's box variants
\** As many cites as you can!
\** Beyaghi \& Cai's survey
\** Combinatorial settings
\* What's missing?
\** Systematic general understanding of existing and to-be-invented variants
\** Example: if we take a variant A box and a variant B box and put them in the same problem, we're stuck!
\* How do we study all of the models at once?
\** CICS framework
\** Variant of bandit superprocesses (forward ref to detailed discussion)
\*/

About CICS:
\* What is CICS?
\** Define it
\** We'll focus on the case of DAG MDPs
\*** Clarify to what extent this is a fundamental limitation
\* Why is CICS hard?
\** Local decisions
\** Global decisions
\** Basically a generalization of MDPs, so no hope of easy solution in general
\* What are we aiming for?
\** Solving CICS by decomposing it into smaller pieces
\** Remarkably, this happens automatically for Markov chain case
\** It's also how most of the progress on Pandora's box variants works
\* What does decomposition mean?
\** Define committing policies, commitment gap, etc.
\* Main questions:
\** How do we understand what commitment gaps are possible?
\** Are there general strategies for constructing low-commitment-gap policies?
\** We ideally want the answers to these questions to also decompose into questions about local arm
\*** E.g. we don't want the commitment for one arm to depend in a very complicated way on all the other arms
\*/

Our contributions:
\* General lower bound strategy/amortization
\** Key idea: \emph{local lower bound}
\** The global bound follows by composing the local lower bounds in a natural way
\** Building on BSP work
\* Methods of designing approximation algorithms for general CICS
\** All based on notions of \emph{local approximation}
\** Key feature: local approximations compose
\*** E.g. if you have a local approximation for a box of variant A and another one for a box of variant B, then you can solve CICS problems with a mix of boxes of both types
\** Building on Laura \& Ziv's work
\*** They work in matroid and other combinatorial settings, not just single-item selection
\* Use local approximation to obtain new approximation results for Pandora's box variants
\** These all come from finding new local approximations
\*/

}
\end{comment}



==> old_introduction.tex <==
\section{Introduction}\label{sec:intro}

Consider a biotechnology company investing in multiple drug discovery projects. Each individual project can involve a multitude of decisions with uncertain outcomes. Typically very few projects will make it to trials and FDA approval at which point they can begin to yield rewards. The company needs to determine how to distribute resources across these projects without knowing upfront which one will succeed and to what extent. Many decision making problems call for upfront investment in information acquisition (such as how much reward a project will generate) before optimizing over multiple options (such as which project to seek FDA approval for). Some other examples include an oil company's search for a good drilling site; a construction company exploring different design ideas for a project; a manufacturer performing market research before determining which products to make and in what quantity, etc.

%1. Weighing scale game. This is a kind of costly information problem.

As a toy example of costly information acquisition in the context of optimization, consider what we call the {\em Weighing Scale} problem. The algorithm is presented with $n$ alternatives with unknown costs, $X_1, \cdots, X_n$, of which it needs to pick a cheap one. Each cost $X_i$ is distributed independently according to a known distribution. The only way the algorithm can learn any further information about the $X_i$'s is to use a weighing scale at the additional cost of $1$ per use: for any index $i$ and target $t$, the weighing scale returns $\mathbbm{1}[X_i \le t]$. What information, if any, should the algorithm gather before making its selection so as to minimize the expected cost of the chosen alternative plus the number of weighings?


In this paper we study a class of problems that we call {\em Costly Information Combinatorial Selection} (henceforth, CICS), of which Weighing Scale is an example. Our goal is to pick a subset of $n$ alternatives with stochastic values satisfying a feasibility constraint. We can obtain information about the value of any individual alternative through a sequence of costly actions tailored to that alternative. In the minimization version of the problem our objective is to minimize the total value of the chosen alternatives plus the cost of information acquisition. In the maximization version we  maximize the total value of the chosen subset minus the cost of information acquisition. 

The algorithmic challenge of CICS stems from two levels of decision-making that influence each other -- which alternative to explore in each step; as well as how to explore the chosen alternative (e.g. which target values $t$ to use in the Weighing Scale setting). A policy can, in general, make these choices adaptively based on the information obtained on previous steps. %These challenges render most variants of the problem computationally hard.

A classic example of the CICS is Weitzman's Pandora's Box problem. Here each alternative is hidden inside a closed box; the goal is to select a single alternative; the algorithm can observe the value of the alternative by opening, a.k.a. ``inspecting'', each box at a cost; and any alternative must be inspected before being selected. Pandora's Box admits an astonishingly simple optimal algorithm: each box is assigned an index based on its cost and value distribution; for minimization, boxes are inspected in increasing\footnote{For the maximization version of the problem, boxes are opened in decreasing order of index.} order of index until the algorithm finds a value that is smaller than all remaining indices and accepts that value. The indices do not depend on the algorithm's stochastic trajectory; the order of information acquisition is therefore non-adaptive. Essentially, {\em the indices capture all of the salient information about each individual box} that can then be used by the algorithm to determine the order in which to explore the boxes. 

Interestingly, this optimality structure extends to a large class of feasibility constraints over Pandora's Boxes: \cite{S17} showed that Weitzman's indices and the corresponding greedy ordering algorithm achieve approximate optimality for essentially all selection problems that admit greedy-style (a.k.a. frugal) approximation algorithms.

%Importantly, indices can be pre-computed and do not depend on the algorithm's stochastic trajectory; the order of information acquisition is therefore non-adaptive. Pandora's Box with combinatorial selection is also by now well understood: \cite{S17} showed that index-based algorithms remain optimal \textcolor{blue}{or near optimal} for a broad class of feasibility constraints -- essentially all selection problems that admit greedy-style exact \textcolor{red}{(why exact?)} algorithms. 

However, the landscape changes if the algorithm has multiple modes of information acquisition available for each alternative. For example, if inspection becomes optional, that is, if the algorithm is allowed to select an alternative without observing its value, the optimal algorithm is no longer non-adaptive and the problem becomes NP-hard. Much effort has been devoted recently towards developing approximations for variants of Pandora's Box, including the optional inspection version and the so-called partial inspection version. See, for example, the survey by \cite{BC24-survey}. These results are generally tailored to the specifics of the variants they study and do not extend to other models of information acquisition. Moreover, they do not always generalize to combinatorial settings.

\begin{center}
\parbox{0.98\textwidth}{
\noindent
A natural question is whether index-based policies can be extended to other CICS settings: can we distill the essence of the information acquisition process for each alternative into a Weitzman-style index, and build an approximation algorithm based on it? This is the question we seek to answer in this paper. }   
\end{center}

%2. Costly information problems have received much attention lately. Pandora's Box as a standard well understood model. Extensions in many directions. Most variants are hard and focus is on approximation. 

%More broadly, in this paper we study combinatorial selection problems where the algorithm aims to select a subset $S$ of the $n$ alternatives satisfying a given feasibility constraint. The algorithm learns information about the alternatives' values through a series of costly actions. We consider both minimization and maximization problems: in the former, the algorithm minimizes the sum of values of the selected alternatives plus the cost spent on learning information. 

We develop a framework for designing approximately-optimal policies for both the minimization and maximization versions of CICS. Our framework has two components. First we develop a bound on the cost of the optimal solution based on a {\bf novel cost amortization technique} that generalizes the Gittins index to Markov Decision Processes. This bound allows us to disentagle the exploration of different alternatives into individual ``local'' problems. We then show that a certain notion of {\bf local approximation} applied to each individual exploration problem can be combined via an index-based policy to obtain a global approximation guarantee. This approach is a strengthening and generalization of the ``Local Hedging'' technique developed by \cite{DS24} in the context of Pandora's Box with optional inspection.

We instantiate our framework with new approximation results for previously studied variants of Pandora's Box as well as the new weighing scale problem described above. Our framework and results extend seamlessly to combinatorial selection problems over matroid constraints as well as to combinations of different variants of information acquisition. For example, when given a selection problem with some weighing-scale-alternatives and some optional-inspection-alternatives, our approach can effortlessly combine local approximations for each variant to obtain a combined guarantee for the whole problem. 

\subsection*{Bandit superprocesses and our cost amortization framework}

%3. More broadly, weighing scale is an example of a bandit superprocess. Results for PB generally focus on the version where there are two or three different actions to take per box. What if there are many many actions and several of them can be taken in sequence? Techniques don't generally scale or provide insight.

Selection problems with costly information are closely related to a class of sequential decision-making problems called bandit superprocesses, which generalize Markovian multi-armed bandits (MAB) \citep{GGW11}. In an MAB, the algorithm is given $n$ Markovian ``arms''; at every step the algorithm can pull any one of the arms and receive a reward; the state of the pulled arm then evolves according to the underlying Markov process. \citet{G79} showed that an index-based policy is optimal for this problem. MAB is usually studied in an infinite horizon setting with discounted or averaged reward. \cite{DTW03} extended this approach to the finite horizon setting (where Markov chains have terminal states) and \cite{GJSS19} further extended it to combinatorial selection. Weitzman's index-policy for Pandora's Box is a special case of these results.

In a general bandit superprocess, the $n$ arms are Markov Decision Processes (MDPs) comprising multiple possible actions with different costs/rewards. While it is possible to treat the superprocess as a single large MDP, the exponential size of this MDP makes this approach computationally infeasible, and it is desirable to consider algorithms that ``solve'' each component process separately and combine the solutions together. \cite{W80} showed that certain bandit superprocesses admit simple index-policies just like the MAB special case. In particular, when each MDP in the superprocess admits an unambiguously optimal static policy, these policies can be composed to obtain a globally optimal policy through appropriately defined indices. However, in the absence of such a strong local optimality condition, the globally optimal policy may take actions that are suboptimal for the MDP they're taken in. \textcolor{blue}{We illustrate such an example in~\Cref{app:example}.}

Much like Whittle's work, our approach considers a local problem $(\mc, y)$ for each MDP $\mc$ where the algorithm is presented with a deterministic outside option $y$ and at any step can either choose to take an action in $\mc$ or accept the outside option $y$. The optimal solution to this local problem generates an optimality curve $\optf_\mc(y)$ as a function of the outside option. A primary technical contribution of our work is to convert this optimality curve into a mapping from terminal states of the MDP to ``surrogate'' costs (Section~\ref{sec:amortization}). The surrogate costs essentially allow an algorithm to amortize the costs of actions and pay (a part of) them only when the MDP terminates. We develop a recursive ``water filling'' algorithm for cost amortization that ensures that good, i.e. low cost or high reward, terminal states are responsible for paying most of the cost share. The overall index of the MDP is then defined to be the cost of the best-case scenario -- the lowest possible surrogate cost that is instantiated. In the special case of Markov chains, our water filling amortization exactly recovers the Gittins index.

A key property of the surrogate costs we define is their {\em independence from the actions chosen} by the algorithm in the MDP (Lemma~\ref{lem:mdp-wf-char-new} in Section~\ref{sec:amortization}). The corresponding indices can therefore be defined and computed independently of the algorithm's stochastic trajectory, much like in Gittins or Weitzman's setting. This allows us to compose these costs and obtain a global bound on the value of the optimal solution. However, the independence comes at a loss -- the surrogate costs provide a bound that is not exact for general MDPs (in contrast to Whittle's results, for example). 

Our approach is heavily influenced by the work of \cite{KWG16} who presented an amortization viewpoint for Weitzman's index for classical Pandora's Box, as well as for its extension to Markov chains. The amortization viewpoint is also implicit in the work of \cite{S17}, who bounds the optimal cost by considering a phantom ``free information'' world. Our amortized cost shares reflect a similar argument. We emphasize that while bounds on the optimal solution's value have been established previously for the single-selection CICS in special cases, a general bound was not known previously. Our bound applies to any feasibility constraint over any bandit superprocess where the constituent MDPs have a DAG-like structure.

\subsection*{Local and semilocal approximation}

Next we consider approximations to the CICS through a class of algorithms called ``commitment policies''. A commitment policy for an instance of the CICS specifies a (random) action for the algorithm to take at any state of any component MDP.\footnote{E.g., in the weighing scale problem, for each $X_i$, we may specify targets $t^i_1, t^i_{11}, t^i_{12},$ etc. such that $X_i$ is first compared against $t^i_1$, and then against $t^i_{11}$ or $t^i_{12}$ depending on whether the first comparison was True or False, and so on and so forth.} The commitment for each alternative depends on its own state and not on the states of other processes. This turns each MDP into a (suboptimal) Markov chain. Armed with these commitments, the algorithm faces a combinatorial MAB which, based on the prior discussion, we know how to solve.

Given the characterization of the optimal cost in terms of properties of the local games $(\mc, y)$ defined above, one reasonable approach is to try to find a commitment policy for each MDP that is approximately optimal for the local game. However, this does not work. Consider, for example, a minimization MDP $\mc$ with two actions. The first action leads to a deterministic value of $1$, and the second leads to a stochastic value of $0$ or $1$ with probability $1/2$ each. Then, the first action provides a $2$-approximation for the local game $(\mc, y)$: its expected cost is $\min(y,1)$ whereas the optimal cost of the local game is half of that quantity, achieved by taking the stochastic option. Now consider a single-selection superprocess with $n$ copies of the above MDP. If we commit to the deterministic action in each MDP, our cost is deterministically $1$, whereas taking the stochastic action in each costs us $1/2^n$ -- an exponential gap!

\cite{DS24} describe how to fix this problem in the context of Pandora's Box with optional inspection and define a local approximation as follows. Let $\optf_\mc(\cdot)$ and $\optf_{\pi}(\cdot)$ denote the optimality curves of the MDP $\mc$ and the commitment policy $\pi$ for $\mc$, respectively, in the local game $(\mc, y)$. The {\em local approximation} factor for minimization achieved by $\pi$ for the MDP $\mc$ is $\alpha\geq 1$ if we have 
\begin{equation}
\label{eq:local}
\optf_\pi(\alpha y)\le \alpha\optf_\mc(y) \,\, \forall y\in \real.
\end{equation}
For maximization, we likewise require $\optf_\pi(\frac y\alpha)\ge \frac 1\alpha \optf_\mc(y)$ for all $y$.
It then holds that any commitment policy that achieves an $\alpha$-local approximation for each constituent MDP achieves a global $\alpha$-approximation.\footnote{Observe that Equation~\eqref{eq:local} is stronger than simply requiring the commitment policy to be approximately optimal for the local game $(\mc, y)$ at every possible outside option $y$ (in other words, $\optf_\pi(y)\le \alpha\optf_\mc(y)$).}  We show in Section~\ref{sec:local_approx} that this composition result holds for general CICS. 

%Local approximation can also be expressed in terms of surrogate costs. Recall that the performance of a commitment policy is related to its surrogate costs, which are different from and typically worse (due to suboptimality in the local game) than the water-filling surrogate costs of the corresponding MDP. 

Informally speaking, local approximation is equivalent to establishing second order stochastic dominance between the surrogate costs of the MDP and the committing policy. We also explore the stronger condition of first order stochastic dominance between surrogate costs, that we call {\em pointwise approximation}, which can be easier to establish in some settings.
%if the two sets of surrogate costs can be related within some factor $\alpha$ for every possible instantiation, then the local approximation factor is bounded by $\alpha$. 
These characterizations allows us to design commitment policies that achieve a good approximation.

%We remark that while bounding the gap between surrogate costs always implies Equation~\eqref{eq:local}, the converse is not true. Nevertheless, we have found both viewpoints to be useful in establishing our approximation results. 

In some settings, the local approximation condition can be challenging to satisfy. For example, if $\optf_\mc$ is near-linear, then Equation~\eqref{eq:local} is essentially equivalent to requiring $\optf_\mc=\optf_\pi$.\footnote{That is, $\pi$ must be unambiguously optimal for $\mc$; and no suboptimal policy can provide any local approximation.} We therefore explore a weakening of the condition by allowing for additive deviations from \eqref{eq:local}. We call this property {\em Semilocal Approximation}, and show that it leads to improved approximation bounds for some settings (Section~\ref{sec:gvo:composition}).

\subsection*{Our results}

We establish new or improved approximation factors for three variants of the CICS. In each case our results apply to matroid feasibility constraints in the given setting. For the first and second settings, our results extend also to feasibility constraints admitting frugal approximation algorithms as defined in \cite{S17}.

\begin{itemize}
    \item {\bf Pandora's Box with Partial Inspection} (\cref{sec:pvo}). This setting is an extension of the classical PB where in addition to opening the box, the algorithm can choose to ``peek'' into the box at a cheaper cost and learn its value; boxes must still be opened before being selected. We consider the minimization version of this problem and present a $\sqrt{2}$-approximation using the notion of local approximation. The minimization version of this problem has not been studied previously.% See Section~\ref{sec:pvo} for details.
    
    \item {\bf Weighing Scale Problem} (\cref{sec:ws}). This is the problem described in the introduction, and is a new problem introduced in this paper. We obtain a logarithmic approximation in key parameters of the problem using the notion of pointwise approximation.% See Section~\ref{sec:ws} for details.

    \item {\bf Pandora's Box with Optional Inspection} (\cref{sec:gvo}). This setting is an extension of the classical PB where the algorithm is allowed to select boxes without opening them. We consider the maximization version of this problem. We show that no committing policy can achieve better than a $0.5$-local approximation. On the other hand, semilocal approximation allows us to achieve a $0.582$-approximation. The maximization version of the problem is extensively studied but previous results only apply to the single selection setting. Our result, in contrast, extends to matroid feasibility constraints.% See Section~\ref{sec:gvo} for details.
    
\end{itemize}
Our cost amortization framework is presented in Section~\ref{sec:amortization} and local approximation in Section~\ref{sec:local_approx}.
A detailed discussion of related work can be found in \Cref{sec:related}.

%Addressed: \textcolor{red}{Dimitris: I think that one thing we are under-selling right now is that we are the first to give a LB for the mdp opt in the \textbf{combinatorial} setting as far as I know. This is also a very good motivating claim for the framework we introduce, as the proof we have immediately extends to combinatorial setting - not sure how this would work with the DP-approach.}





%%%%%%%%%%%%%
 
CICS relates to bandit superprocesses (BSPs), introduced by \citet{N73}, where multiple independent MDPs evolve as the algorithm advances one at each step, receiving a (discounted) reward. Unlike BSPs, a CICS algorithm must terminate by selecting a feasible set, and its MDPs, modeling information acquisition, are acyclic. Our techniques rely on this acyclicity, whereas BSPs can involve general MDPs.

When BSPs reduce to Markov chains, they become the well-studied Multi-Armed Bandit (MAB) problem, which admits a simple optimal policy \citep{G79}: each state in a Markov chain has an independent index, and the algorithm advances the chain with the highest index. This extends to finite-horizon settings \citep{DTW03}, with \citet{W79}'s PB algorithm as a special case.

General BSPs lack indexability \citep{G82}, but \citet{W80} developed a bounding approach via a local problem $(\mc, y)$, where an algorithm either advances an MDP $\mc$ or terminates at cost $y$. The optimality curve $\optf_\mc(y)$ acts as a surrogate cost distribution, forming the Whittle integral \citep{W80,BS13}.

Our work transforms this optimality curve into surrogate costs mapped to terminal states, allowing cost amortization through a recursive ``water filling'' algorithm. This ensures lower-cost terminal states bear more cost. A key property is that surrogate cost distributions remain independent of algorithmic choices, enabling global composition. In the Markov chain case, our amortization exactly recovers the Gittins index for MAB.

Our approach builds on \citet{KWG16}, who framed Weitzman’s index as an amortization argument, and \citet{S17}, who analyzed optimal cost bounds via a ``free information'' world. Our method generalizes these ideas to finite-horizon MDPs under arbitrary combinatorial constraints.


==> proof_backup.tex <==

The rest of this section is dedicated towards proving~\Cref{lem:mdp-wf-char}. Fix any MDP $\mc=(S, \sigma, A, c, \dist, V, T)$. The proof follows by \textit{induction on the horizon} $H$ of the MDP, i.e. the maximum number of actions required to terminate $\mc$. If $H=1$, then $\mc$ must correspond to a (single) terminal state $\sigma\in T$. In that case, the only committing policy in $\comset{\mc}$ is to accept the value of $\sigma$, and setting $W(\sigma)=v(\sigma)$ trivially satisfies the conditions of the lemma. From now on, we assume that~\Cref{lem:mdp-wf-char} holds for all MDPs of horizon up to $H$ and will prove it for an MDP $\mc$ of horizon $H+1$.

Let $\mc$ be of horizon $H+1$ and let $A(\sigma)=\{a_1,\cdots , a_k\}$ be the set of actions available at the starting state $\sigma$. For each $i\in [k]$, let $\mc_i$ denote the subprocess of $\mc$ that starts in state $\sigma$, has \textbf{only} action $a_i$ available and then proceeds exactly as $\mc$. Note that each MDP $\mc_i$ is also an MDP of horizon $H+1$. We use $T_i$ to denote the terminal states of $\mc_i$; from the tree-like structure of $\mc$, note that $\{T_i\}_{i=1}^k$ is a partition of $T$. We break the proof in two steps; first we will use the induction hypothesis to show that the lemma holds for each $\mc_i$ separately, and then we will combine the guarantees for each $\mc_i$ to prove the lemma for $\mc$.


\paragraph{Step 1.} We consider the MDP $\mc_i$ for some $i\in [k]$. We use $R_i$ to denote the set of all states of $\mc_i$ that can be reached directly by taking action $a_i$ on $\sigma$; that is, $R_i:=\{s\in S: \dist(\sigma, a_i, s) > 0\}$. For each $s\in R_i$, we use $\mc_s$ to denote the subprocesses of $\mc_i$ that is rooted on state $s$. In other words, a trajectory in $\mc_i$ corresponds to taking action $a_i$, realizing a set $s\in R_i$ and then taking a trajectory in $\mc_s$. 

By the inductive properties of optimality curves, we have
\begin{align*}
    \optf_{\mc_i}(y) &= \min\bigg( y , c(a_i) + \sum_{s\in R_i}\dist(\sigma,a_i,s)\cdot f_{\mc_s}(y)\bigg) \\
    &= \min\bigg( y , c(a_i) + \sum_{s\in R_i}\dist(\sigma,a_i,s)\cdot \expect{\min\{y, W^*_{\mc_s}\}}\bigg)  && \text{(By~\Cref{def:mdp-wf})} \\
   &= \min\bigg( y , c(a_i) + \expect{\min\{y , Z_i\}} \bigg) 
\end{align*}
where $Z_i$ corresponds to the random variable obtained by first sampling a state $s\in R_i$ from $\dist(\sigma, a_i , \cdot)$ and then sampling from $W^*_{\mc_s}$. Now, let $g_i$ be the solution to equation
\[c(a_i) + \expect{\min\{y , Z_i\}} = \expect{\min\{y , \max(g_i, Z_i)\}}\]
or equivalently the minimum value in the support of the random variable we obtain after performing a water-filling amortization of the cost $c(a_i)$ onto $Z_i$. Then, we have that $f_{\mc_i}(y) = \expect{\min\{y, \max(g_i,Z_i)\}}$ and by~\Cref{def:mdp-wf} this implies that $W^*_{\mc_i} = \max(g_i, Z_i)$.

For each $s\in R_i$, the MDP $\mc_s$ has horizon at most $H$ by construction. Thus, there exist mappings $W_s(\cdot)$ over the terminals $T(s)$ that satisfy the action independence and cost dominance properties. For each $t\in T_i$, let $Z_i(t)$ denote the distribution $W_s(t)$ for the unique $s\in R_i$ such that $t\in T(s)$. We now define the mapping of~\Cref{lem:mdp-wf-char} for $\mc_i$ to be
\[W(t) := \max(g_i , Z_i(t))\]

We will now prove that this mapping $W(\cdot)$ satisfies action independence. Consider any committing policy $\pi\in\comset{\mc_i}$. Since $\mc_i$ has only action $a_i$ available at its root, $\pi$ corresponds to a set $\{\pi_s\}$ of committing policies over the MDPs $\mc_s$. Thus, sampling a terminal $t\in p_\pi$ and then sampling from $W(t)$ is equivalent to sampling a state $s\in R_i$, then sampling a terminal $t\sim p_{\pi_s}$, then sampling from distribution $W_s(t)$ and finally return the maximum of the sampled cost and $g_i$. Since $W_s(\cdot )$ satisfy action independence, this is equivalent to sampling a state $s\in R_i$, then sampling a cost from $W^*_{\mc_s}$ and returning the maximum of the cost in $g_i$; since $W^*_{\mc_i} = \max(g_i, Z_i)$, this is equivalent to directly sampling from $W^*_{\mc_i}$, proving action independence. 

\textcolor{red}{Need to think how to write cost dominance a little  more, the proof is getting very long.}

\paragraph{Step 2.} We have shown that the lemma holds for all subprocesses $\mc_i$, resulting to mappings $W_i(\cdot)$ on their terminal states $T_i$. We will now prove that it will also hold for $\mc$. Note that for any fixed outside option $y$, we have the following principle of optimality:
\[\optf_\mc(y) = \min\left\{y, \min_{i\in [k]} \optf_{\mc_i}(y)\right\}.\]
By~\Cref{def:mdp-wf}, we can re-write this as $\expect{\min\{y, W^*_\mc \}} = \min_{i\in [k]}\left\{\expect{\min\{y, W^*_{\mc_i}\}} \right\}$ and thus conclude that $\expect{\min\{ y, W^*_\mc\}} \leq \expect{\min \{y, W^*_{\mc_i}\}}$ for all $i\in [k]$. This allows us to use the following technical lemma, whose proof is involved and deferred to~\Cref{app:amortization}.



\begin{lemma}[Stochastic Dominance Lemma]\label{lemma:sdom}
Let $X, Z$ be any two discrete random variables that satisfy the property $\expect{\min\{y, X\}} \leq \expect{\min\{y, Z\}}$ for all $y\in\real$. There exists a mapping $m: \mathrm{supp}(Z) \mapsto \Delta(\mathrm{supp}(X))$ from the support of $Z$ to distributions over the support of $X$ such that:
\begin{enumerate}
    \item $X$ is obtained by sampling from $m(z)$ for a randomly sampled $z\sim Z$.
    \item For all $z\in\mathrm{support}(Z)$, it holds that $\expect{m(z)}\leq z$.
\end{enumerate}
\end{lemma}

We apply~\Cref{lemma:sdom} to all tuples $(W^*_\mc , W^*_{\mc_i})$ of surrogate costs to obtain mappings $m_i(\cdot)$. Now, for each $t\in T$, let $i(t)\in [k]$ be the index $i$ of the unique subprocess $\mc_i$ such that $t\in T_i$. The mapping $W(t)$ of~\Cref{lem:mdp-wf-char} for $\mc$ is given by first sampling a number $z$ from distribution $W_{i(t)}(t)$ and then sampling from $m_{i(t)}(z)$. We immediately obtain that this mapping $W(\cdot)$ satisfies both the action independence condition and the cost dominance condition by the inductive hypothesis on $W_i(\cdot)$ combined with the properties of the mappings $m_i(\cdot)$ due to~\Cref{lemma:sdom}, concluding the proof.

==> structure.tex <==
\subsection{Paper Structure}
\Dimitris{The purpose of this section is to figure out what, how and in which order to present our main results, in other words it should contain (semi)-final versions of all our definitions, notation and main theorem statements. Once we figure this out, we can decide how to present these in the paper. I am breaking this in three sections; one for our general MDP framework, one for extensions of it and one for the applications we will consider.}


\subsection{The Superprocess Framework}


We begin by giving a formal, inductive definition of a \textit{superprocess}, as superprocesses will be the central object of interest in this work.

\begin{definition}[Superprocess]
    We distinguish between trivial and non-trivial superprocesses. A trivial superprocess $P$ is characterized by a single value $v_P\geq 0$. A non-trivial superprocess $P$ is characterized by a non-empty set of actions $A(P)$; each action $a\in A(P)$ is described by an action cost $c_a\geq 0$ and a distribution $D_a$ over both trivial and non-trivial superprocesses $P'\in\supp{D_a}$. 
\end{definition}


Next, we proceed to define \textit{Markov chains}, a very important sub-class of superprocesses where all the action sets have a cardinality of one.
\begin{definition}[Markov Chain]
    Every trivial superprocess is a Markov chain. A non-trivial superprocess $P$ is a Markov chain if it has a unique action (i.e. $A(P)=\{a\}$) and each $P'\in\supp{D_a}$ is a Markov chain.
\end{definition}

Up next, we define the central optimization problem that this work studies. Initially, an algorithm is presented with some number $n$ of superprocesses, and needs to decide which one to \textit{advance}; advancing a superprocess $P$ corresponds to selecting one of its actions $a\in A(P)$ by paying the corresponding cost $c_a$, and then letting nature independently realize a new superprocess $P'\in\supp{D_a}$ to substitute $P$ with. If at any point the realizations result to a trivial superprocess $P$, the algorithm also has the option of paying its cost $v_P$ to terminate the game. Formally:


\begin{definition}[Superprocess Game]
    A superprocess game $SG=(P_1,\dotsc ,P_n)$ is an optimization problem whose input consists of $n\geq 1$ superprocesses $P_i$. A feasible policy $\pi$ for $SG$ is an algorithm that must select between (i) picking any trivial (if any) superprocess $P_i$ and paying its cost $v_{P_i}$, or (ii) picking any non-trivial (if any) superprocess $P_i$ and an action $a\in A(P_i)$, paying the action cost $c_a$ and then proceed to play $SG'=(P'_1,\dotsc ,P'_n)$ where $P'_i$ is a randomly realized superprocess from $D_a$ and $P'_j=P_j$ for all $j\neq i$.
\end{definition}

In other words, a policy $\pi$ corresponds to a (perhaps random) protocol that determines for each possible state of the game whether to pick a realized trivial superprocess, pay its cost and terminate or whether to pick a non-trivial superprocess, advance it through one of its actions by paying the associated cost and then continue to play the game on the randomly realized outcome. We use $\pi(SG)$ to denote the expected total cost of the policy on instance $SG$ over the randomness of the superprocess realizations as well as the randomness of the policy. We use $\opt (SG)$ to denote the minimum policy cost for instance $SG$. Clearly, the optimal policy for a superprocess game is well-defined, but it is not clear whether characterizing it is even computationally tractable. The aim of this work is to determine sufficient conditions under which one can hope to compute or approximate this optimal policy. 

As a first step, consider the special case of a superprocess game whose input consists of just a superprocess $P$ and a \textit{trivial} superprocess $Q$ of cost $v_{Q}=y$ for some $y\geq 0$. Then, any policy for this simple game needs to decide whether it is worth it to advance $P$ through one of its actions or simply pay the cost of $y$ to terminate. We will use $f_P(y)$ to denote the optimal cost of this game as a function of $y$, and will refer to this as the optimality curve for superprocess $P$:

\begin{definition}[Optimality Curves]
    For any superprocess $P$ and any number $y\geq 0$, let $Q_y$ denote the trivial superprocess of value $y$ and $SG_y$ denote the superprocess game on input $(P,Q_y)$.
    Then, we define the optimality curve of superprocess $P$ as the function $f_P(y):= \opt (SG_y)$.
\end{definition}

As it turns out, we are able to encode the optimality curve of any superprocess $P$ through a random variable $W_P$ which we refer to as the \textit{surrogate cost} of $P$. This is a consequence of the fact for any superprocess $P$, the optimality curve $f_P(y)$ is a continuous, concave function dominated by the $g(y)=y$ line, and thus $1-f'_P(y)$ is a valid cumulative distribution function.

\begin{claim}[Surrogate Cost]
    For any superprocess $P$ with optimality curve $f_P(\cdot)$, there exists a random variable $W_P$ (which we refer to as $P$'s surrogate cost) such that $f_P(y) = \mathbb{E}[\min(y,W_P)]$ for all $y\geq 0$. 
\end{claim}

While these surrogate costs simply capture the optimal cost for a superprocess game with a single superprocess $P$ and a termination option $y$, it turns out that they provide us with enough information to lower bound the optimal cost on arbitrary superprocess games.

\begin{lemma}[Surrogate Cost Lower Bound]
    For any superprocess game $SG=(P_1,\dotsc , P_n)$, it holds that \[\opt (SG) \geq \mathbb{E}[\min_{i\in [n]}W_{P_i}].\] 
    In the special case where $P_i$ is a Markov chain for all $i\in [n]$, the above holds with equality.
\end{lemma}


We comment that the above result was already known for both Markov chains \textit{and} superprocesses in settings similar to ours. However, we provide a novel proof of these results that does not depend on the definition of surrogate costs through optimality curves (like previous approaches did), but instead recovers them naturally, through an intuitive amortization argument. Furthermore, this novel approach allows us to recover the optimal policy for the special case of Markov chains through the lenses of amortization.

\begin{lemma}[Optimal Policy for Markov Chains]
    For the special case of a superprocess game $SG$ on Markov chains, there exists an efficient policy that achieves the optimal cost.
\end{lemma}

\Dimitris{Not sure how to write this yet.} At this point, we need to comment on our notion of \textit{efficiency}. One could imagine of enumerating all the possible policies for a superprocess game, but it is not even clear if doing so is computationally tractable. On the other hand, if the game consisted of a single Markov chain $P$ and a termination option $y$, the critical values for terminating would correspond to some combination of the advancement costs and the trivial superprocess values that are descendants of $P$; in that sense, one could identify the optimal policy in time polynomial to the \say{size} of $P$. However, applying the same approach to games with multiple superprocesses would require time polynomial to the product of their sizes. An efficient policy would instead depend on the sum of their sizes; in other words, an efficient policy requires as much work for a superprocess game as it would for a single superprocess (with termination option) game. \Dimitris{This whole paragraph to be changed, i.e. come up with a formal notion of efficiency.}



Up next, we turn our attention to superprocesses that are not Markov chains. Far less results are known in this setting, and one of our main contributions is to provide a sufficient condition under which we can efficiently approximate the optimal policy. The main computational barrier is that a policy does not only need to decide which superprocess to advance, but also through which of its actions. It has been observed that this significantly complicates the structure of the optimal policy, making the underlying problem much harder.

To circumvent these computational issues, a natural approach would be to only consider \textit{committing} policies, i.e. policies that whenever they advance a superprocess $P$ they will always do it through the same action $a\in A(P)$, no matter the state of the other superprocesses. 

\begin{definition}[Committing Policy]
    A commitment $C$ is defined with respect to a superprocess $P$ and corresponds to a unique action $a\in A(P)$, as well as a unique action $a'\in A(P')$ for all superprocesses $P'$ that are \say{generated} by $P$ (meaning there is a sequence of advancements on $P$ that potentially results to $P'$). A committing policy with respect to $C$ is a policy for superprocess games that include $P$ and whenever $P$ (or a generated superprocess) gets advances, it is always done so by the committing action. We use $f_{P|C}(y)$ to denote the cost of the optimal policy that respects $C$ in the superprocess game $(P,Q_y)$.
\end{definition}


One could think of a commitment as \textit{pruning} the action spaces of the underlying superprocesses until each of them is reduced to a Markov chain. Then, conditioned on a specific commitment, we can use our results on Markov chains to determine an efficient policy that is optimal, subject to the commitment. However, it is not clear whether there exists some specific commitment for which the underlying optimal policy is a good approximation to the overall optimal. For example, past results on approximating the superprocess game have assumed that for each $(P,Q_y)$ game there exists an optimal committing policy (this is known as Whittle's condition) and under this assumption one can indeed characterize an efficient optimal solution to the superprocess game.

Beyond this assumption, very few results are known. Recent work on a specific version of the superprocess game introduced the notion of local approximation as a sufficient condition for settings where Whittle's condition doesn't hold. We will now re-introduce this property for general superprocess games.

\begin{definition}[Local Approximation]
    We say that a superprocess $P$ admits a $\alpha$-local approximation for some $\alpha\geq 1$ if there exists some distribution $\Delta$ over commitments $C$ with respect to $P$ such that
    \[\mathbb{E}_{C\sim\Delta}[f_{P|C}(y)]\leq \alpha\cdot f_P(\frac{y}{\alpha}).\]
\end{definition}

With this, we are now ready to state our main theorem.

\begin{theorem}
    Consider any superprocess game $SG=(P_1,\dotsc , P_n)$. Then, if every $P_i$ admits an $\alpha$-local approximation, there exists an efficient policy that $\alpha$-approximates the optimal policy. 
\end{theorem}

\Dimitris{Mention the algorithm (hedging), efficiency of finding probabilities and multi-mdp to single-mdp complexity reduction.}


\subsection{Extensions}
\begin{enumerate}
    \item We prove all of our results for discrete and finite superprocesses. We do this for ease of exposition, here we show that all the arguments can be extended to both continuous distributions and infinite (i.e. with loops) superprocesses.

    \item Maximization. One could think that instead of paying the leaf cost, we instead get rewarded with its value. This results in a mixed signed objective (selected value - action costs). We show that all of our arguments continue to work in this setting.

    \item Multi-Process selection. This is something we should probably mention much earlier; while the surrogate cost lower bound was known, our amortization based proof allows us to easily extend it in much more general settings such as matroid constraints. \textcolor{blue}{Will add more details on this once we figure it out.}
\end{enumerate}


\subsection{Applications}


\begin{enumerate}
    \item Peek vs Open.
    \item \Dimitris{Need more...}
\end{enumerate}
